Surprisingly Strong Performance Prediction with Neural Graph Features

Performance prediction has been a key part of the neural architecture search (NAS) process, allowing to speed up NAS algorithms by avoiding resource-consuming network training. Although many performance predictors correlate well with ground truth performance, they require training data in the form of trained networks. Recently, zero-cost proxies have been proposed as an efficient method to estimate network performance without any training. However, they are still poorly understood, exhibit biases with network properties, and their performance is limited. Inspired by the drawbacks of zero-cost proxies, we propose neural graph features (GRAF), simple to compute properties of architectural graphs. GRAF offers fast and interpretable performance prediction while outperforming zero-cost proxies and other common encodings. In combination with other zero-cost proxies, GRAF outperforms most existing performance predictors at a fraction of the cost.

==> brpnas_tables.tex <==
\begin{table}
\small
\addtolength{\tabcolsep}{-0.2em}
\centering
\caption{BRP-NAS model results on the APGD-CE adversarial accuracy prediction tasks for different $\epsilon$ values. Average and standard deviation of Kendall's tau over 50 independent runs.}
\vskip 0.15in\begin{tabular}{r|ccc|ccc|ccc}
 & \multicolumn{3}{|c}{aa\_apgd-ce@Linf\_eps-0.1} & \multicolumn{3}{|c}{aa\_apgd-ce@Linf\_eps-0.5} & \multicolumn{3}{|c}{aa\_apgd-ce@Linf\_eps-1.0} \\
 & 32 & 128 & 1024 & 32 & 128 & 1024 & 32 & 128 & 1024 \\
\hline
None & $0.49^{0.04}$ & $0.58^{0.04}$ & $0.79^{0.02}$ & $0.15^{0.08}$ & $0.28^{0.05}$ & $0.60^{0.01}$ & $0.20^{0.09}$ & $0.43^{0.07}$ & $0.69^{0.01}$ \\
Onehot & $0.52^{0.05}$ & $0.63^{0.03}$ & $0.78^{0.02}$ & $0.16^{0.07}$ & $0.28^{0.05}$ & $0.60^{0.01}$ & $0.21^{0.07}$ & $0.44^{0.07}$ & $0.69^{0.01}$ \\
GRAF & $0.57^{0.06}$ & $0.68^{0.01}$ & $0.78^{0.01}$ & $0.19^{0.07}$ & \boldmath $0.31^{0.04}$ & $0.56^{0.06}$ & $0.25^{0.07}$ & $0.43^{0.04}$ & $0.68^{0.02}$ \\
Onehot + F\&P & $0.56^{0.03}$ & $0.64^{0.03}$ & $0.77^{0.02}$ & $0.16^{0.05}$ & $0.29^{0.05}$ & $0.61^{0.01}$ & $0.23^{0.06}$ & $0.44^{0.06}$ & $0.69^{0.01}$ \\
GRAF + Onehot & $0.58^{0.05}$ & $0.67^{0.02}$ & $0.78^{0.01}$ & $0.19^{0.07}$ & $0.30^{0.03}$ & $0.52^{0.07}$ & $0.26^{0.06}$ & $0.42^{0.05}$ & $0.67^{0.04}$ \\
GRAF + F\&P & $0.59^{0.04}$ & $0.68^{0.02}$ & $0.77^{0.01}$ & \boldmath $0.20^{0.05}$ & $0.29^{0.03}$ & $0.54^{0.07}$ & $0.25^{0.06}$ & $0.41^{0.05}$ & $0.68^{0.02}$ \\
GRAF + Onehot + F\&P & $0.57^{0.05}$ & $0.67^{0.02}$ & $0.78^{0.01}$ & $0.19^{0.08}$ & $0.30^{0.03}$ & $0.52^{0.07}$ & $0.25^{0.06}$ & $0.39^{0.06}$ & $0.67^{0.04}$ \\
\hline
ZCP + F\&P & $0.62^{0.04}$ & $0.66^{0.02}$ & $0.79^{0.01}$ & $0.16^{0.06}$ & $0.28^{0.05}$ & $0.61^{0.01}$ & $0.21^{0.07}$ & \boldmath $0.44^{0.07}$ & \boldmath $0.70^{0.01}$ \\
ZCP + Onehot + F\&P & \boldmath $0.63^{0.03}$ & $0.68^{0.02}$ & $0.78^{0.01}$ & $0.16^{0.05}$ & $0.29^{0.05}$ & \boldmath $0.61^{0.01}$ & $0.25^{0.06}$ & $0.42^{0.06}$ & $0.69^{0.01}$ \\
ZCP + GRAF + F\&P & $0.61^{0.04}$ & \boldmath $0.70^{0.02}$ & $0.80^{0.01}$ & $0.19^{0.07}$ & $0.29^{0.05}$ & $0.57^{0.05}$ & \boldmath $0.27^{0.06}$ & $0.43^{0.06}$ & $0.68^{0.02}$ \\
Everything & $0.61^{0.05}$ & $0.70^{0.01}$ & \boldmath $0.80^{0.01}$ & $0.20^{0.05}$ & $0.30^{0.03}$ & $0.55^{0.06}$ & $0.26^{0.07}$ & $0.42^{0.06}$ & $0.69^{0.01}$ \\
\end{tabular}\end{table}\begin{table}
\small
\addtolength{\tabcolsep}{-0.2em}
\centering
\caption{BRP-NAS model results on the Square adversarial accuracy prediction tasks for different $\epsilon$ values. Average and standard deviation of Kendall's tau over 50 independent runs.}
\vskip 0.15in\begin{tabular}{r|ccc|ccc|ccc}
 & \multicolumn{3}{|c}{aa\_square@Linf\_eps-0.1} & \multicolumn{3}{|c}{aa\_square@Linf\_eps-0.5} & \multicolumn{3}{|c}{aa\_square@Linf\_eps-1.0} \\
 & 32 & 128 & 1024 & 32 & 128 & 1024 & 32 & 128 & 1024 \\
\hline
None & $0.49^{0.06}$ & $0.59^{0.04}$ & $0.81^{0.02}$ & $0.43^{0.05}$ & $0.56^{0.05}$ & \boldmath $0.75^{0.01}$ & $0.28^{0.06}$ & $0.39^{0.04}$ & $0.61^{0.02}$ \\
Onehot & $0.55^{0.06}$ & $0.65^{0.02}$ & $0.80^{0.02}$ & $0.47^{0.06}$ & $0.59^{0.03}$ & $0.75^{0.01}$ & $0.30^{0.04}$ & $0.41^{0.04}$ & $0.61^{0.02}$ \\
GRAF & $0.63^{0.04}$ & $0.71^{0.02}$ & $0.80^{0.01}$ & $0.53^{0.05}$ & $0.63^{0.02}$ & $0.72^{0.01}$ & $0.34^{0.06}$ & $0.42^{0.03}$ & $0.55^{0.03}$ \\
Onehot + F\&P & $0.58^{0.04}$ & $0.66^{0.02}$ & $0.79^{0.02}$ & $0.51^{0.04}$ & $0.60^{0.02}$ & $0.75^{0.02}$ & $0.31^{0.05}$ & $0.42^{0.02}$ & $0.60^{0.02}$ \\
GRAF + Onehot & $0.60^{0.04}$ & $0.71^{0.02}$ & $0.80^{0.01}$ & $0.53^{0.04}$ & $0.62^{0.02}$ & $0.73^{0.02}$ & $0.31^{0.05}$ & $0.43^{0.02}$ & $0.56^{0.03}$ \\
GRAF + F\&P & $0.62^{0.03}$ & $0.70^{0.01}$ & $0.80^{0.01}$ & $0.55^{0.04}$ & $0.63^{0.02}$ & $0.72^{0.02}$ & $0.33^{0.06}$ & $0.42^{0.02}$ & $0.56^{0.04}$ \\
GRAF + Onehot + F\&P & $0.61^{0.04}$ & $0.70^{0.02}$ & $0.80^{0.01}$ & $0.53^{0.04}$ & $0.62^{0.02}$ & $0.73^{0.02}$ & $0.33^{0.05}$ & $0.43^{0.02}$ & $0.56^{0.03}$ \\
\hline
ZCP + F\&P & $0.65^{0.05}$ & $0.68^{0.02}$ & $0.81^{0.02}$ & $0.56^{0.05}$ & $0.61^{0.02}$ & $0.75^{0.02}$ & $0.34^{0.05}$ & $0.42^{0.03}$ & \boldmath $0.61^{0.02}$ \\
ZCP + Onehot + F\&P & $0.65^{0.03}$ & $0.71^{0.02}$ & $0.82^{0.01}$ & $0.55^{0.03}$ & $0.63^{0.02}$ & $0.75^{0.02}$ & $0.32^{0.06}$ & $0.42^{0.03}$ & $0.60^{0.02}$ \\
ZCP + GRAF + F\&P & \boldmath $0.66^{0.05}$ & \boldmath $0.73^{0.02}$ & $0.83^{0.01}$ & \boldmath $0.57^{0.05}$ & $0.64^{0.02}$ & $0.74^{0.01}$ & $0.33^{0.07}$ & \boldmath $0.44^{0.02}$ & $0.56^{0.03}$ \\
Everything & $0.63^{0.05}$ & $0.73^{0.02}$ & \boldmath $0.83^{0.01}$ & $0.55^{0.04}$ & \boldmath $0.64^{0.02}$ & $0.75^{0.01}$ & \boldmath $0.35^{0.05}$ & $0.42^{0.02}$ & $0.56^{0.03}$ \\
\end{tabular}\end{table}\begin{table}
\small
\addtolength{\tabcolsep}{-0.2em}
\centering
\caption{BRP-NAS model results on the FGSM adversarial accuracy prediction tasks for different $\epsilon$ values. Average and standard deviation of Kendall's tau over 50 independent runs.}
\vskip 0.15in\begin{tabular}{r|ccc|ccc|ccc}
 & \multicolumn{3}{|c}{fgsm@Linf\_eps-0.1} & \multicolumn{3}{|c}{fgsm@Linf\_eps-0.5} & \multicolumn{3}{|c}{fgsm@Linf\_eps-1.0} \\
 & 32 & 128 & 1024 & 32 & 128 & 1024 & 32 & 128 & 1024 \\
\hline
None & $0.48^{0.05}$ & $0.58^{0.04}$ & $0.80^{0.01}$ & $0.42^{0.07}$ & $0.55^{0.03}$ & $0.74^{0.01}$ & $0.44^{0.06}$ & $0.60^{0.03}$ & $0.78^{0.01}$ \\
Onehot & $0.53^{0.05}$ & $0.64^{0.03}$ & $0.78^{0.02}$ & $0.44^{0.05}$ & $0.55^{0.04}$ & $0.74^{0.01}$ & $0.47^{0.06}$ & $0.60^{0.02}$ & $0.79^{0.01}$ \\
GRAF & $0.60^{0.04}$ & $0.69^{0.02}$ & $0.78^{0.02}$ & $0.50^{0.04}$ & $0.58^{0.02}$ & $0.69^{0.03}$ & $0.54^{0.05}$ & $0.62^{0.02}$ & $0.77^{0.03}$ \\
Onehot + F\&P & $0.56^{0.04}$ & $0.65^{0.02}$ & $0.78^{0.02}$ & $0.45^{0.05}$ & $0.57^{0.02}$ & $0.74^{0.01}$ & $0.48^{0.05}$ & $0.61^{0.02}$ & $0.79^{0.01}$ \\
GRAF + Onehot & $0.58^{0.04}$ & $0.68^{0.02}$ & $0.79^{0.01}$ & $0.47^{0.06}$ & $0.58^{0.02}$ & $0.70^{0.02}$ & $0.54^{0.04}$ & $0.62^{0.02}$ & $0.77^{0.03}$ \\
GRAF + F\&P & $0.61^{0.05}$ & $0.69^{0.02}$ & $0.78^{0.01}$ & $0.48^{0.06}$ & $0.58^{0.01}$ & $0.69^{0.02}$ & \boldmath $0.55^{0.05}$ & $0.62^{0.02}$ & $0.77^{0.03}$ \\
GRAF + Onehot + F\&P & $0.59^{0.05}$ & $0.68^{0.02}$ & $0.78^{0.02}$ & $0.49^{0.05}$ & $0.58^{0.02}$ & $0.69^{0.02}$ & $0.53^{0.05}$ & \boldmath $0.62^{0.02}$ & $0.76^{0.04}$ \\
\hline
ZCP + F\&P & $0.62^{0.04}$ & $0.67^{0.02}$ & $0.80^{0.01}$ & $0.48^{0.06}$ & $0.56^{0.03}$ & \boldmath $0.74^{0.01}$ & $0.50^{0.04}$ & $0.61^{0.03}$ & $0.79^{0.01}$ \\
ZCP + Onehot + F\&P & $0.62^{0.04}$ & $0.68^{0.02}$ & $0.79^{0.01}$ & $0.48^{0.04}$ & $0.58^{0.02}$ & $0.74^{0.01}$ & $0.51^{0.06}$ & $0.62^{0.02}$ & \boldmath $0.79^{0.01}$ \\
ZCP + GRAF + F\&P & \boldmath $0.63^{0.04}$ & \boldmath $0.71^{0.02}$ & $0.80^{0.02}$ & \boldmath $0.50^{0.05}$ & \boldmath $0.59^{0.01}$ & $0.70^{0.02}$ & $0.55^{0.06}$ & $0.62^{0.02}$ & $0.77^{0.02}$ \\
Everything & $0.62^{0.03}$ & $0.71^{0.02}$ & \boldmath $0.81^{0.01}$ & $0.49^{0.05}$ & $0.59^{0.01}$ & $0.70^{0.02}$ & $0.54^{0.04}$ & $0.62^{0.02}$ & $0.77^{0.03}$ \\
\end{tabular}\end{table}\begin{table}
\small
\addtolength{\tabcolsep}{-0.2em}
\centering
\caption{BRP-NAS model results on the PGD adversarial accuracy prediction tasks for different $\epsilon$ values. Average and standard deviation of Kendall's tau over 50 independent runs.}
\vskip 0.15in\begin{tabular}{r|ccc|ccc|ccc}
 & \multicolumn{3}{|c}{pgd@Linf\_eps-0.1} & \multicolumn{3}{|c}{pgd@Linf\_eps-0.5} & \multicolumn{3}{|c}{pgd@Linf\_eps-1.0} \\
 & 32 & 128 & 1024 & 32 & 128 & 1024 & 32 & 128 & 1024 \\
\hline
None & $0.48^{0.05}$ & $0.58^{0.05}$ & $0.79^{0.02}$ & $0.24^{0.07}$ & $0.36^{0.04}$ & $0.61^{0.01}$ & $0.21^{0.06}$ & $0.37^{0.06}$ & $0.68^{0.01}$ \\
Onehot & $0.53^{0.04}$ & $0.64^{0.03}$ & $0.78^{0.02}$ & $0.24^{0.06}$ & $0.37^{0.03}$ & $0.61^{0.02}$ & $0.22^{0.07}$ & $0.36^{0.05}$ & $0.68^{0.01}$ \\
GRAF & $0.61^{0.04}$ & $0.69^{0.02}$ & $0.78^{0.01}$ & $0.28^{0.07}$ & $0.39^{0.02}$ & $0.55^{0.03}$ & $0.28^{0.05}$ & $0.39^{0.04}$ & $0.66^{0.04}$ \\
Onehot + F\&P & $0.56^{0.03}$ & $0.65^{0.02}$ & $0.78^{0.02}$ & $0.25^{0.07}$ & $0.36^{0.03}$ & $0.60^{0.02}$ & $0.24^{0.05}$ & $0.38^{0.05}$ & $0.68^{0.01}$ \\
GRAF + Onehot & $0.59^{0.04}$ & $0.68^{0.02}$ & $0.79^{0.01}$ & $0.29^{0.05}$ & $0.39^{0.02}$ & $0.54^{0.04}$ & $0.27^{0.06}$ & $0.39^{0.04}$ & $0.66^{0.04}$ \\
GRAF + F\&P & $0.60^{0.05}$ & $0.69^{0.01}$ & $0.79^{0.01}$ & $0.28^{0.08}$ & $0.39^{0.02}$ & $0.53^{0.03}$ & $0.27^{0.07}$ & $0.39^{0.03}$ & $0.66^{0.05}$ \\
GRAF + Onehot + F\&P & $0.60^{0.05}$ & $0.68^{0.02}$ & $0.79^{0.01}$ & \boldmath $0.31^{0.04}$ & $0.39^{0.02}$ & $0.54^{0.03}$ & $0.25^{0.09}$ & $0.38^{0.03}$ & $0.65^{0.05}$ \\
\hline
ZCP + F\&P & $0.64^{0.04}$ & $0.67^{0.02}$ & $0.80^{0.02}$ & $0.25^{0.07}$ & $0.37^{0.03}$ & \boldmath $0.61^{0.02}$ & $0.24^{0.06}$ & $0.38^{0.04}$ & $0.68^{0.01}$ \\
ZCP + Onehot + F\&P & $0.63^{0.04}$ & $0.68^{0.02}$ & $0.79^{0.01}$ & $0.26^{0.06}$ & $0.37^{0.03}$ & $0.61^{0.02}$ & $0.25^{0.06}$ & $0.38^{0.05}$ & \boldmath $0.69^{0.01}$ \\
ZCP + GRAF + F\&P & \boldmath $0.64^{0.04}$ & \boldmath $0.72^{0.02}$ & $0.80^{0.01}$ & $0.30^{0.06}$ & \boldmath $0.40^{0.03}$ & $0.55^{0.03}$ & \boldmath $0.30^{0.07}$ & \boldmath $0.40^{0.04}$ & $0.66^{0.04}$ \\
Everything & $0.62^{0.04}$ & $0.71^{0.02}$ & \boldmath $0.81^{0.01}$ & $0.28^{0.06}$ & $0.39^{0.03}$ & $0.55^{0.03}$ & $0.27^{0.07}$ & $0.40^{0.04}$ & $0.66^{0.05}$ \\
\end{tabular}\end{table}\begin{table}
\small
\addtolength{\tabcolsep}{-0.2em}
\centering
\caption{BRP-NAS model results on the energy consumption prediction tasks. Average and standard deviation of Kendall's tau over 50 independent runs.}
\vskip 0.15in\begin{tabular}{r|ccc|ccc|ccc}
 & \multicolumn{3}{|c}{edgegpu\_energy} & \multicolumn{3}{|c}{eyeriss\_energy} & \multicolumn{3}{|c}{fpga\_energy} \\
 & 32 & 128 & 1024 & 32 & 128 & 1024 & 32 & 128 & 1024 \\
\hline
None & $0.59^{0.05}$ & $0.71^{0.01}$ & $0.80^{0.00}$ & $0.78^{0.03}$ & $0.89^{0.01}$ & $0.96^{0.00}$ & $0.85^{0.03}$ & $0.94^{0.01}$ & $0.98^{0.00}$ \\
Onehot & $0.67^{0.05}$ & $0.77^{0.01}$ & $0.87^{0.00}$ & $0.86^{0.04}$ & $0.95^{0.01}$ & \boldmath $0.99^{0.00}$ & $0.85^{0.03}$ & $0.95^{0.01}$ & $0.98^{0.00}$ \\
GRAF & $0.75^{0.03}$ & $0.81^{0.01}$ & $0.86^{0.00}$ & $0.82^{0.03}$ & $0.94^{0.01}$ & $0.98^{0.00}$ & $0.93^{0.01}$ & $0.96^{0.00}$ & $0.99^{0.00}$ \\
Onehot + F\&P & $0.69^{0.04}$ & $0.78^{0.01}$ & $0.87^{0.00}$ & \boldmath $0.89^{0.02}$ & \boldmath $0.95^{0.01}$ & $0.99^{0.00}$ & $0.87^{0.02}$ & $0.95^{0.01}$ & $0.99^{0.00}$ \\
GRAF + Onehot & \boldmath $0.77^{0.03}$ & $0.83^{0.01}$ & $0.87^{0.00}$ & $0.80^{0.04}$ & $0.93^{0.01}$ & $0.98^{0.00}$ & $0.94^{0.01}$ & $0.97^{0.00}$ & $0.99^{0.00}$ \\
GRAF + F\&P & $0.75^{0.02}$ & $0.82^{0.01}$ & $0.86^{0.00}$ & $0.82^{0.03}$ & $0.94^{0.01}$ & $0.99^{0.00}$ & $0.94^{0.01}$ & $0.96^{0.00}$ & \boldmath $0.99^{0.00}$ \\
GRAF + Onehot + F\&P & $0.77^{0.02}$ & \boldmath $0.83^{0.01}$ & \boldmath $0.87^{0.00}$ & $0.80^{0.04}$ & $0.93^{0.01}$ & $0.98^{0.00}$ & \boldmath $0.95^{0.01}$ & \boldmath $0.98^{0.00}$ & $0.99^{0.00}$ \\
\hline
ZCP + F\&P & $0.63^{0.05}$ & $0.72^{0.01}$ & $0.81^{0.00}$ & $0.80^{0.04}$ & $0.90^{0.01}$ & $0.97^{0.00}$ & $0.87^{0.03}$ & $0.95^{0.01}$ & $0.98^{0.00}$ \\
ZCP + Onehot + F\&P & $0.71^{0.04}$ & $0.78^{0.01}$ & $0.87^{0.00}$ & $0.80^{0.05}$ & $0.94^{0.02}$ & $0.99^{0.00}$ & $0.88^{0.02}$ & $0.95^{0.01}$ & $0.98^{0.00}$ \\
ZCP + GRAF + F\&P & $0.74^{0.03}$ & $0.81^{0.01}$ & $0.86^{0.00}$ & $0.77^{0.04}$ & $0.93^{0.01}$ & $0.98^{0.00}$ & $0.93^{0.02}$ & $0.96^{0.01}$ & $0.99^{0.00}$ \\
Everything & $0.75^{0.04}$ & $0.83^{0.01}$ & $0.87^{0.00}$ & $0.76^{0.05}$ & $0.92^{0.01}$ & $0.98^{0.00}$ & $0.94^{0.02}$ & $0.97^{0.00}$ & $0.99^{0.00}$ \\
\end{tabular}\end{table}\begin{table}
\small
\addtolength{\tabcolsep}{-0.2em}
\centering
\caption{BRP-NAS model results on the latency prediction tasks. Average and standard deviation of Kendall's tau over 50 independent runs.}
\vskip 0.15in\begin{tabular}{r|ccc|ccc|ccc}
 & \multicolumn{3}{|c}{edgegpu\_latency} & \multicolumn{3}{|c}{edgetpu\_latency} & \multicolumn{3}{|c}{eyeriss\_latency} \\
 & 32 & 128 & 1024 & 32 & 128 & 1024 & 32 & 128 & 1024 \\
\hline
None & $0.59^{0.05}$ & $0.72^{0.01}$ & $0.80^{0.00}$ & $0.59^{0.08}$ & $0.69^{0.04}$ & \boldmath $0.84^{0.02}$ & $0.80^{0.03}$ & $0.91^{0.01}$ & $0.96^{0.00}$ \\
Onehot & $0.73^{0.04}$ & $0.83^{0.01}$ & \boldmath $0.87^{0.00}$ & $0.55^{0.13}$ & $0.73^{0.04}$ & $0.83^{0.02}$ & $0.84^{0.03}$ & $0.92^{0.01}$ & $0.96^{0.00}$ \\
GRAF & $0.73^{0.04}$ & $0.82^{0.01}$ & $0.87^{0.00}$ & $0.49^{0.16}$ & $0.73^{0.04}$ & $0.81^{0.02}$ & $0.92^{0.01}$ & $0.95^{0.00}$ & $0.96^{0.00}$ \\
Onehot + F\&P & $0.74^{0.03}$ & $0.83^{0.01}$ & $0.87^{0.00}$ & $0.56^{0.12}$ & \boldmath $0.73^{0.04}$ & $0.83^{0.02}$ & $0.85^{0.03}$ & $0.93^{0.01}$ & $0.96^{0.00}$ \\
GRAF + Onehot & $0.75^{0.03}$ & \boldmath $0.83^{0.01}$ & $0.87^{0.00}$ & $0.41^{0.15}$ & $0.72^{0.04}$ & $0.81^{0.02}$ & $0.92^{0.02}$ & $0.96^{0.00}$ & $0.96^{0.00}$ \\
GRAF + F\&P & $0.73^{0.03}$ & $0.82^{0.01}$ & $0.87^{0.00}$ & $0.44^{0.16}$ & $0.73^{0.03}$ & $0.81^{0.02}$ & $0.92^{0.01}$ & $0.95^{0.00}$ & $0.96^{0.00}$ \\
GRAF + Onehot + F\&P & \boldmath $0.75^{0.04}$ & $0.83^{0.01}$ & $0.87^{0.00}$ & $0.42^{0.14}$ & $0.72^{0.04}$ & $0.81^{0.02}$ & \boldmath $0.92^{0.01}$ & \boldmath $0.96^{0.00}$ & \boldmath $0.96^{0.00}$ \\
\hline
ZCP + F\&P & $0.62^{0.05}$ & $0.72^{0.01}$ & $0.81^{0.00}$ & \boldmath $0.60^{0.09}$ & $0.70^{0.04}$ & $0.83^{0.02}$ & $0.79^{0.04}$ & $0.91^{0.01}$ & $0.95^{0.00}$ \\
ZCP + Onehot + F\&P & $0.72^{0.05}$ & $0.83^{0.01}$ & $0.87^{0.00}$ & $0.47^{0.13}$ & $0.72^{0.04}$ & $0.82^{0.02}$ & $0.82^{0.04}$ & $0.92^{0.01}$ & $0.95^{0.00}$ \\
ZCP + GRAF + F\&P & $0.69^{0.05}$ & $0.82^{0.01}$ & $0.87^{0.00}$ & $0.45^{0.12}$ & $0.72^{0.03}$ & $0.81^{0.02}$ & $0.90^{0.02}$ & $0.95^{0.00}$ & $0.96^{0.00}$ \\
Everything & $0.72^{0.05}$ & $0.82^{0.01}$ & $0.87^{0.00}$ & $0.41^{0.16}$ & $0.71^{0.04}$ & $0.81^{0.02}$ & $0.90^{0.02}$ & $0.95^{0.00}$ & $0.96^{0.00}$ \\
\end{tabular}\end{table}\begin{table}
\small
\addtolength{\tabcolsep}{-0.2em}
\centering
\caption{BRP-NAS model results on the latency prediction tasks. Average and standard deviation of Kendall's tau over 50 independent runs.}
\vskip 0.15in\begin{tabular}{r|ccc|ccc|ccc}
 & \multicolumn{3}{|c}{fpga\_latency} & \multicolumn{3}{|c}{pixel3\_latency} & \multicolumn{3}{|c}{raspi4\_latency} \\
 & 32 & 128 & 1024 & 32 & 128 & 1024 & 32 & 128 & 1024 \\
\hline
None & $0.85^{0.03}$ & $0.94^{0.01}$ & $0.98^{0.00}$ & $0.73^{0.04}$ & $0.83^{0.01}$ & $0.88^{0.00}$ & $0.73^{0.05}$ & $0.83^{0.01}$ & $0.87^{0.00}$ \\
Onehot & $0.86^{0.03}$ & $0.95^{0.01}$ & $0.99^{0.00}$ & $0.75^{0.03}$ & $0.83^{0.01}$ & $0.88^{0.00}$ & $0.75^{0.03}$ & $0.84^{0.01}$ & $0.87^{0.00}$ \\
GRAF & $0.93^{0.02}$ & $0.98^{0.00}$ & \boldmath $0.99^{0.00}$ & $0.81^{0.02}$ & $0.84^{0.01}$ & $0.89^{0.00}$ & $0.81^{0.02}$ & $0.84^{0.01}$ & $0.87^{0.00}$ \\
Onehot + F\&P & $0.92^{0.02}$ & $0.96^{0.01}$ & $0.99^{0.00}$ & $0.76^{0.03}$ & $0.83^{0.01}$ & $0.88^{0.00}$ & $0.76^{0.03}$ & $0.84^{0.01}$ & $0.87^{0.00}$ \\
GRAF + Onehot & $0.93^{0.02}$ & $0.98^{0.00}$ & $0.99^{0.00}$ & $0.81^{0.02}$ & $0.85^{0.01}$ & \boldmath $0.89^{0.00}$ & $0.82^{0.02}$ & $0.85^{0.01}$ & $0.87^{0.00}$ \\
GRAF + F\&P & \boldmath $0.94^{0.01}$ & \boldmath $0.98^{0.00}$ & $0.99^{0.00}$ & \boldmath $0.82^{0.02}$ & $0.85^{0.01}$ & $0.89^{0.00}$ & $0.82^{0.02}$ & $0.85^{0.01}$ & $0.87^{0.00}$ \\
GRAF + Onehot + F\&P & $0.94^{0.01}$ & $0.98^{0.00}$ & $0.99^{0.00}$ & $0.82^{0.02}$ & \boldmath $0.85^{0.01}$ & $0.89^{0.00}$ & \boldmath $0.82^{0.02}$ & \boldmath $0.85^{0.01}$ & \boldmath $0.88^{0.00}$ \\
\hline
ZCP + F\&P & $0.91^{0.02}$ & $0.95^{0.01}$ & $0.99^{0.00}$ & $0.73^{0.04}$ & $0.83^{0.01}$ & $0.88^{0.00}$ & $0.75^{0.03}$ & $0.83^{0.01}$ & $0.87^{0.00}$ \\
ZCP + Onehot + F\&P & $0.91^{0.02}$ & $0.96^{0.01}$ & $0.99^{0.00}$ & $0.74^{0.03}$ & $0.83^{0.01}$ & $0.88^{0.00}$ & $0.76^{0.03}$ & $0.83^{0.01}$ & $0.87^{0.00}$ \\
ZCP + GRAF + F\&P & $0.91^{0.03}$ & $0.98^{0.00}$ & $0.99^{0.00}$ & $0.80^{0.03}$ & $0.84^{0.01}$ & $0.89^{0.00}$ & $0.81^{0.02}$ & $0.85^{0.01}$ & $0.87^{0.00}$ \\
Everything & $0.91^{0.03}$ & $0.98^{0.00}$ & $0.99^{0.00}$ & $0.81^{0.02}$ & $0.85^{0.01}$ & $0.89^{0.00}$ & $0.82^{0.02}$ & $0.85^{0.01}$ & $0.87^{0.00}$ \\
\end{tabular}\end{table}\begin{table}
\small
\addtolength{\tabcolsep}{-0.2em}
\centering
\caption{BRP-NAS model results on the arithmetic intensity and validation accuracy prediction tasks. Average and standard deviation of Kendall's tau over 50 independent runs.}
\vskip 0.15in\begin{tabular}{r|ccc|ccc|ccc}
 & \multicolumn{3}{|c}{eyeriss\_arithmetic\_intensity} & \multicolumn{3}{|c}{val\_accs} & \multicolumn{3}{|c}{imagenet\_val\_accs} \\
 & 32 & 128 & 1024 & 32 & 128 & 1024 & 32 & 128 & 1024 \\
\hline
None & $0.68^{0.06}$ & $0.89^{0.01}$ & $0.96^{0.00}$ & $0.48^{0.05}$ & $0.58^{0.04}$ & $0.80^{0.02}$ & $0.48^{0.06}$ & $0.61^{0.03}$ & $0.84^{0.01}$ \\
Onehot & $0.73^{0.06}$ & $0.90^{0.01}$ & $0.96^{0.00}$ & $0.53^{0.05}$ & $0.63^{0.02}$ & $0.77^{0.02}$ & $0.54^{0.04}$ & $0.63^{0.02}$ & $0.83^{0.01}$ \\
GRAF & $0.82^{0.03}$ & $0.92^{0.01}$ & $0.97^{0.00}$ & $0.62^{0.04}$ & $0.69^{0.01}$ & $0.79^{0.01}$ & $0.62^{0.04}$ & $0.69^{0.02}$ & $0.83^{0.01}$ \\
Onehot + F\&P & $0.77^{0.05}$ & $0.91^{0.01}$ & $0.96^{0.00}$ & $0.57^{0.04}$ & $0.64^{0.02}$ & $0.77^{0.02}$ & $0.54^{0.04}$ & $0.64^{0.02}$ & $0.83^{0.02}$ \\
GRAF + Onehot & $0.82^{0.03}$ & \boldmath $0.93^{0.01}$ & $0.97^{0.00}$ & $0.59^{0.05}$ & $0.69^{0.02}$ & $0.79^{0.01}$ & $0.61^{0.04}$ & $0.69^{0.02}$ & $0.83^{0.01}$ \\
GRAF + F\&P & \boldmath $0.83^{0.02}$ & $0.92^{0.01}$ & $0.97^{0.00}$ & $0.62^{0.03}$ & $0.69^{0.02}$ & $0.78^{0.01}$ & $0.62^{0.03}$ & $0.69^{0.02}$ & $0.83^{0.01}$ \\
GRAF + Onehot + F\&P & $0.82^{0.03}$ & $0.93^{0.01}$ & \boldmath $0.97^{0.00}$ & $0.61^{0.04}$ & $0.69^{0.02}$ & $0.79^{0.01}$ & $0.61^{0.04}$ & $0.68^{0.02}$ & $0.83^{0.02}$ \\
\hline
ZCP + F\&P & $0.77^{0.03}$ & $0.90^{0.01}$ & $0.96^{0.00}$ & $0.63^{0.03}$ & $0.66^{0.02}$ & $0.80^{0.02}$ & $0.56^{0.04}$ & $0.63^{0.03}$ & \boldmath $0.85^{0.01}$ \\
ZCP + Onehot + F\&P & $0.79^{0.03}$ & $0.91^{0.01}$ & $0.96^{0.00}$ & $0.64^{0.04}$ & $0.68^{0.02}$ & $0.79^{0.01}$ & $0.58^{0.03}$ & $0.66^{0.02}$ & $0.83^{0.02}$ \\
ZCP + GRAF + F\&P & $0.81^{0.03}$ & $0.92^{0.01}$ & $0.97^{0.00}$ & \boldmath $0.65^{0.05}$ & $0.72^{0.02}$ & \boldmath $0.81^{0.01}$ & \boldmath $0.64^{0.03}$ & \boldmath $0.71^{0.02}$ & $0.84^{0.01}$ \\
Everything & $0.80^{0.04}$ & $0.92^{0.01}$ & $0.97^{0.00}$ & $0.64^{0.04}$ & \boldmath $0.72^{0.02}$ & $0.81^{0.01}$ & $0.63^{0.03}$ & $0.71^{0.02}$ & $0.84^{0.01}$ \\
\end{tabular}\end{table}

==> hw_tables.tex <==
\begin{table}
    \small
    \addtolength{\tabcolsep}{-0.2em}
    \centering
    \caption{Results on the {\tt fpga\_energy} task for various datasets. Average and standard deviation of Kendall tau over 50 independent runs. Bold values indicate the best results and those that are not statistically different from them. \label{ap:tab:fpgaen}}
    \vskip 0.15in
    \begin{tabular}{r|ccc|ccc|ccc}
dataset & \multicolumn{3}{|c}{cifar10} & \multicolumn{3}{|c}{cifar100} & \multicolumn{3}{|c}{ImageNet16-120} \\
train\_size & 32 & 128 & 1024 & 32 & 128 & 1024 & 32 & 128 & 1024 \\
\hline
OH & $0.55^{0.07}$ & $0.72^{0.04}$ & $0.85^{0.00}$ & $0.55^{0.07}$ & $0.72^{0.04}$ & $0.85^{0.00}$ & $0.58^{0.08}$ & $0.74^{0.03}$ & $0.89^{0.00}$ \\
OH + FP & $0.83^{0.02}$ & $0.89^{0.01}$ & $0.97^{0.00}$ & $0.83^{0.02}$ & $0.89^{0.01}$ & $0.97^{0.00}$ & $\mathbf{0.90^{0.02}}$ & $0.95^{0.00}$ & $0.99^{0.00}$ \\
GRAF & $0.81^{0.04}$ & $\mathbf{0.95^{0.01}}$ & $\mathbf{1.00^{0.00}}$ & $0.81^{0.04}$ & $\mathbf{0.95^{0.01}}$ & $\mathbf{1.00^{0.00}}$ & $0.85^{0.05}$ & $\mathbf{0.96^{0.01}}$ & $\mathbf{1.00^{0.00}}$ \\
GRAF + FP & $\mathbf{0.85^{0.02}}$ & $0.94^{0.01}$ & $1.00^{0.00}$ & $\mathbf{0.85^{0.02}}$ & $0.94^{0.01}$ & $1.00^{0.00}$ & $\mathbf{0.89^{0.03}}$ & $\mathbf{0.96^{0.00}}$ & $1.00^{0.00}$ \\
GRAF + OH & $0.81^{0.03}$ & $0.95^{0.01}$ & $\mathbf{1.00^{0.00}}$ & $0.81^{0.03}$ & $0.95^{0.01}$ & $\mathbf{1.00^{0.00}}$ & $0.85^{0.04}$ & $\mathbf{0.96^{0.01}}$ & $\mathbf{1.00^{0.00}}$ \\
GRAF + OH + FP & $\mathbf{0.85^{0.02}}$ & $0.94^{0.01}$ & $1.00^{0.00}$ & $\mathbf{0.85^{0.02}}$ & $0.94^{0.01}$ & $1.00^{0.00}$ & $\mathbf{0.88^{0.03}}$ & $\mathbf{0.96^{0.00}}$ & $1.00^{0.00}$ \\
\hline
ZCP & $0.82^{0.02}$ & $0.88^{0.01}$ & $0.96^{0.00}$ & $0.82^{0.02}$ & $0.88^{0.01}$ & $0.96^{0.00}$ & $0.88^{0.02}$ & $0.94^{0.00}$ & $0.98^{0.00}$ \\
ZCP + OH & $0.82^{0.02}$ & $0.88^{0.01}$ & $0.96^{0.00}$ & $0.82^{0.02}$ & $0.88^{0.01}$ & $0.96^{0.00}$ & $0.88^{0.02}$ & $0.94^{0.00}$ & $0.98^{0.00}$ \\
ZCP + GRAF & $\mathbf{0.84^{0.03}}$ & $0.93^{0.01}$ & $0.99^{0.00}$ & $\mathbf{0.85^{0.03}}$ & $0.93^{0.01}$ & $0.99^{0.00}$ & $\mathbf{0.89^{0.03}}$ & $0.96^{0.01}$ & $0.99^{0.00}$ \\
ZCP + GRAF + OH & $0.84^{0.03}$ & $0.93^{0.01}$ & $0.99^{0.00}$ & $0.84^{0.03}$ & $0.93^{0.01}$ & $0.99^{0.00}$ & $\mathbf{0.89^{0.03}}$ & $0.96^{0.01}$ & $1.00^{0.00}$ \\
\end{tabular}
    \end{table}\begin{table}
    \small
    \addtolength{\tabcolsep}{-0.2em}
    \centering
    \caption{Results on the {\tt fpga\_latency} task for various datasets. Average and standard deviation of Kendall tau over 50 independent runs. Bold values indicate the best results and those that are not statistically different from them. \label{ap:tab:fpgalat}}
    \vskip 0.15in
    \begin{tabular}{r|ccc|ccc|ccc}
dataset & \multicolumn{3}{|c}{cifar10} & \multicolumn{3}{|c}{cifar100} & \multicolumn{3}{|c}{ImageNet16-120} \\
train\_size & 32 & 128 & 1024 & 32 & 128 & 1024 & 32 & 128 & 1024 \\
\hline
OH & $0.55^{0.07}$ & $0.72^{0.03}$ & $0.85^{0.00}$ & $0.55^{0.07}$ & $0.72^{0.03}$ & $0.85^{0.00}$ & $0.58^{0.08}$ & $0.74^{0.03}$ & $0.89^{0.00}$ \\
OH + FP & $0.83^{0.02}$ & $0.89^{0.01}$ & $0.97^{0.00}$ & $0.83^{0.02}$ & $0.89^{0.01}$ & $0.97^{0.00}$ & $\mathbf{0.90^{0.02}}$ & $0.95^{0.00}$ & $0.99^{0.00}$ \\
GRAF & $0.81^{0.04}$ & $0.95^{0.01}$ & $\mathbf{1.00^{0.00}}$ & $0.81^{0.04}$ & $0.95^{0.01}$ & $\mathbf{1.00^{0.00}}$ & $0.85^{0.05}$ & $\mathbf{0.96^{0.01}}$ & $\mathbf{1.00^{0.00}}$ \\
GRAF + FP & $\mathbf{0.85^{0.02}}$ & $0.94^{0.01}$ & $1.00^{0.00}$ & $\mathbf{0.85^{0.02}}$ & $0.94^{0.01}$ & $1.00^{0.00}$ & $\mathbf{0.89^{0.03}}$ & $\mathbf{0.96^{0.00}}$ & $1.00^{0.00}$ \\
GRAF + OH & $0.81^{0.04}$ & $\mathbf{0.95^{0.01}}$ & $\mathbf{1.00^{0.00}}$ & $0.81^{0.04}$ & $\mathbf{0.95^{0.01}}$ & $\mathbf{1.00^{0.00}}$ & $0.85^{0.04}$ & $\mathbf{0.96^{0.01}}$ & $\mathbf{1.00^{0.00}}$ \\
GRAF + OH + FP & $\mathbf{0.85^{0.02}}$ & $0.94^{0.01}$ & $1.00^{0.00}$ & $\mathbf{0.85^{0.02}}$ & $0.94^{0.01}$ & $1.00^{0.00}$ & $\mathbf{0.88^{0.03}}$ & $\mathbf{0.96^{0.00}}$ & $1.00^{0.00}$ \\
\hline
ZCP & $0.82^{0.02}$ & $0.88^{0.01}$ & $0.96^{0.00}$ & $0.82^{0.02}$ & $0.88^{0.01}$ & $0.96^{0.00}$ & $0.88^{0.02}$ & $0.94^{0.00}$ & $0.98^{0.00}$ \\
ZCP + OH & $0.82^{0.02}$ & $0.88^{0.01}$ & $0.96^{0.00}$ & $0.82^{0.02}$ & $0.88^{0.01}$ & $0.96^{0.00}$ & $0.88^{0.02}$ & $0.94^{0.00}$ & $0.98^{0.00}$ \\
ZCP + GRAF & $\mathbf{0.84^{0.03}}$ & $0.93^{0.01}$ & $0.99^{0.00}$ & $\mathbf{0.84^{0.03}}$ & $0.93^{0.01}$ & $0.99^{0.00}$ & $\mathbf{0.89^{0.03}}$ & $0.96^{0.01}$ & $1.00^{0.00}$ \\
ZCP + GRAF + OH & $0.84^{0.03}$ & $0.93^{0.01}$ & $0.99^{0.00}$ & $\mathbf{0.84^{0.03}}$ & $0.93^{0.01}$ & $0.99^{0.00}$ & $\mathbf{0.89^{0.03}}$ & $0.96^{0.01}$ & $1.00^{0.00}$ \\
\end{tabular}
    \end{table}\begin{table}
    \small
    \addtolength{\tabcolsep}{-0.2em}
    \centering
    \caption{Results on the {\tt eyeriss\_arithmetic\_intensity} task for various datasets. Average and standard deviation of Kendall tau over 50 independent runs. Bold values indicate the best results and those that are not statistically different from them. \label{ap:tab:eyerissar}}
    \vskip 0.15in
    \begin{tabular}{r|ccc|ccc|ccc}
dataset & \multicolumn{3}{|c}{cifar10} & \multicolumn{3}{|c}{cifar100} & \multicolumn{3}{|c}{ImageNet16-120} \\
train\_size & 32 & 128 & 1024 & 32 & 128 & 1024 & 32 & 128 & 1024 \\
\hline
OH & $0.53^{0.08}$ & $0.73^{0.04}$ & $0.88^{0.01}$ & $0.53^{0.08}$ & $0.73^{0.04}$ & $0.88^{0.01}$ & $0.53^{0.08}$ & $0.73^{0.04}$ & $0.88^{0.01}$ \\
OH + FP & $0.65^{0.04}$ & $0.77^{0.02}$ & $0.94^{0.01}$ & $0.65^{0.04}$ & $0.77^{0.02}$ & $0.94^{0.01}$ & $0.64^{0.04}$ & $0.76^{0.03}$ & $0.92^{0.01}$ \\
GRAF & $\mathbf{0.78^{0.05}}$ & $\mathbf{0.92^{0.01}}$ & $\mathbf{0.99^{0.00}}$ & $\mathbf{0.78^{0.05}}$ & $0.92^{0.01}$ & $\mathbf{0.99^{0.00}}$ & $0.78^{0.05}$ & $\mathbf{0.93^{0.01}}$ & $\mathbf{1.00^{0.00}}$ \\
GRAF + FP & $\mathbf{0.78^{0.05}}$ & $0.91^{0.02}$ & $0.99^{0.00}$ & $\mathbf{0.78^{0.05}}$ & $0.91^{0.02}$ & $0.99^{0.00}$ & $\mathbf{0.79^{0.05}}$ & $0.93^{0.02}$ & $\mathbf{1.00^{0.00}}$ \\
GRAF + OH & $\mathbf{0.78^{0.05}}$ & $\mathbf{0.92^{0.02}}$ & $\mathbf{0.99^{0.00}}$ & $\mathbf{0.78^{0.05}}$ & $\mathbf{0.92^{0.02}}$ & $0.99^{0.00}$ & $0.78^{0.05}$ & $\mathbf{0.93^{0.01}}$ & $\mathbf{1.00^{0.00}}$ \\
GRAF + OH + FP & $\mathbf{0.78^{0.05}}$ & $0.91^{0.02}$ & $0.99^{0.00}$ & $\mathbf{0.78^{0.05}}$ & $0.91^{0.02}$ & $0.99^{0.00}$ & $\mathbf{0.79^{0.05}}$ & $0.93^{0.02}$ & $1.00^{0.00}$ \\
\hline
ZCP & $0.61^{0.04}$ & $0.72^{0.02}$ & $0.88^{0.00}$ & $0.61^{0.04}$ & $0.72^{0.02}$ & $0.88^{0.01}$ & $0.62^{0.03}$ & $0.70^{0.01}$ & $0.85^{0.01}$ \\
ZCP + OH & $0.63^{0.04}$ & $0.74^{0.02}$ & $0.89^{0.00}$ & $0.63^{0.04}$ & $0.74^{0.02}$ & $0.89^{0.00}$ & $0.64^{0.03}$ & $0.73^{0.02}$ & $0.88^{0.01}$ \\
ZCP + GRAF & $0.75^{0.05}$ & $0.89^{0.02}$ & $0.99^{0.00}$ & $0.75^{0.05}$ & $0.89^{0.02}$ & $0.99^{0.00}$ & $\mathbf{0.78^{0.04}}$ & $0.91^{0.02}$ & $0.99^{0.00}$ \\
ZCP + GRAF + OH & $0.75^{0.05}$ & $0.89^{0.02}$ & $0.99^{0.00}$ & $0.75^{0.05}$ & $0.89^{0.02}$ & $0.99^{0.00}$ & $\mathbf{0.78^{0.04}}$ & $0.91^{0.02}$ & $0.99^{0.00}$ \\
\end{tabular}
    \end{table}\begin{table}
    \small
    \addtolength{\tabcolsep}{-0.2em}
    \centering
    \caption{Results on the {\tt eyeriss\_energy} task for various datasets. Average and standard deviation of Kendall tau over 50 independent runs. Bold values indicate the best results and those that are not statistically different from them. \label{ap:tab:eyerissen}}
    \vskip 0.15in
    \begin{tabular}{r|ccc|ccc|ccc}
dataset & \multicolumn{3}{|c}{cifar10} & \multicolumn{3}{|c}{cifar100} & \multicolumn{3}{|c}{ImageNet16-120} \\
train\_size & 32 & 128 & 1024 & 32 & 128 & 1024 & 32 & 128 & 1024 \\
\hline
OH & $0.48^{0.06}$ & $0.67^{0.05}$ & $0.84^{0.01}$ & $0.48^{0.06}$ & $0.67^{0.05}$ & $0.84^{0.01}$ & $0.48^{0.06}$ & $0.67^{0.05}$ & $0.84^{0.01}$ \\
OH + FP & $0.61^{0.04}$ & $0.76^{0.03}$ & $0.90^{0.01}$ & $0.62^{0.04}$ & $0.76^{0.03}$ & $0.90^{0.01}$ & $0.62^{0.04}$ & $0.76^{0.03}$ & $0.90^{0.01}$ \\
GRAF & $0.87^{0.03}$ & $0.97^{0.00}$ & $\mathbf{1.00^{0.00}}$ & $0.87^{0.04}$ & $0.97^{0.00}$ & $\mathbf{1.00^{0.00}}$ & $\mathbf{0.87^{0.03}}$ & $0.97^{0.00}$ & $1.00^{0.00}$ \\
GRAF + FP & $\mathbf{0.87^{0.04}}$ & $\mathbf{0.97^{0.00}}$ & $\mathbf{1.00^{0.00}}$ & $\mathbf{0.88^{0.04}}$ & $\mathbf{0.97^{0.00}}$ & $\mathbf{1.00^{0.00}}$ & $\mathbf{0.87^{0.04}}$ & $\mathbf{0.97^{0.00}}$ & $\mathbf{1.00^{0.00}}$ \\
GRAF + OH & $0.87^{0.04}$ & $0.97^{0.00}$ & $\mathbf{1.00^{0.00}}$ & $0.86^{0.04}$ & $0.97^{0.00}$ & $\mathbf{1.00^{0.00}}$ & $0.87^{0.04}$ & $0.97^{0.00}$ & $1.00^{0.00}$ \\
GRAF + OH + FP & $\mathbf{0.87^{0.03}}$ & $\mathbf{0.97^{0.00}}$ & $\mathbf{1.00^{0.00}}$ & $\mathbf{0.87^{0.03}}$ & $0.97^{0.00}$ & $\mathbf{1.00^{0.00}}$ & $\mathbf{0.87^{0.04}}$ & $0.97^{0.00}$ & $\mathbf{1.00^{0.00}}$ \\
\hline
ZCP & $0.56^{0.05}$ & $0.68^{0.02}$ & $0.84^{0.01}$ & $0.55^{0.05}$ & $0.68^{0.02}$ & $0.84^{0.01}$ & $0.53^{0.07}$ & $0.67^{0.02}$ & $0.85^{0.01}$ \\
ZCP + OH & $0.59^{0.05}$ & $0.71^{0.03}$ & $0.84^{0.01}$ & $0.59^{0.05}$ & $0.71^{0.03}$ & $0.84^{0.01}$ & $0.57^{0.07}$ & $0.71^{0.03}$ & $0.84^{0.01}$ \\
ZCP + GRAF & $\mathbf{0.88^{0.04}}$ & $\mathbf{0.97^{0.00}}$ & $1.00^{0.00}$ & $\mathbf{0.88^{0.04}}$ & $\mathbf{0.97^{0.00}}$ & $1.00^{0.00}$ & $\mathbf{0.87^{0.04}}$ & $\mathbf{0.97^{0.00}}$ & $1.00^{0.00}$ \\
ZCP + GRAF + OH & $\mathbf{0.87^{0.04}}$ & $\mathbf{0.97^{0.00}}$ & $1.00^{0.00}$ & $\mathbf{0.87^{0.04}}$ & $\mathbf{0.97^{0.00}}$ & $1.00^{0.00}$ & $\mathbf{0.87^{0.04}}$ & $\mathbf{0.97^{0.00}}$ & $1.00^{0.00}$ \\
\end{tabular}
    \end{table}\begin{table}
    \small
    \addtolength{\tabcolsep}{-0.2em}
    \centering
    \caption{Results on the {\tt eyeriss\_latency} task for various datasets. Average and standard deviation of Kendall tau over 50 independent runs. Bold values indicate the best results and those that are not statistically different from them. \label{ap:tab:eyerisslat}}
    \vskip 0.15in
    \begin{tabular}{r|ccc|ccc|ccc}
dataset & \multicolumn{3}{|c}{cifar10} & \multicolumn{3}{|c}{cifar100} & \multicolumn{3}{|c}{ImageNet16-120} \\
train\_size & 32 & 128 & 1024 & 32 & 128 & 1024 & 32 & 128 & 1024 \\
\hline
OH & $0.49^{0.06}$ & $0.67^{0.04}$ & $0.84^{0.01}$ & $0.49^{0.06}$ & $0.68^{0.04}$ & $0.84^{0.01}$ & $0.49^{0.06}$ & $0.67^{0.04}$ & $0.84^{0.01}$ \\
OH + FP & $0.56^{0.04}$ & $0.72^{0.03}$ & $0.90^{0.01}$ & $0.56^{0.04}$ & $0.72^{0.03}$ & $0.91^{0.01}$ & $0.56^{0.04}$ & $0.72^{0.03}$ & $0.90^{0.01}$ \\
GRAF & $\mathbf{0.88^{0.04}}$ & $\mathbf{0.96^{0.00}}$ & $\mathbf{0.99^{0.00}}$ & $\mathbf{0.88^{0.04}}$ & $\mathbf{0.97^{0.00}}$ & $\mathbf{0.99^{0.00}}$ & $\mathbf{0.88^{0.03}}$ & $\mathbf{0.96^{0.00}}$ & $\mathbf{0.99^{0.00}}$ \\
GRAF + FP & $\mathbf{0.88^{0.04}}$ & $\mathbf{0.96^{0.00}}$ & $\mathbf{0.99^{0.00}}$ & $\mathbf{0.88^{0.04}}$ & $\mathbf{0.97^{0.00}}$ & $\mathbf{0.99^{0.00}}$ & $\mathbf{0.88^{0.04}}$ & $\mathbf{0.96^{0.00}}$ & $\mathbf{0.99^{0.00}}$ \\
GRAF + OH & $\mathbf{0.88^{0.04}}$ & $\mathbf{0.96^{0.00}}$ & $\mathbf{0.99^{0.00}}$ & $\mathbf{0.88^{0.04}}$ & $\mathbf{0.97^{0.00}}$ & $\mathbf{0.99^{0.00}}$ & $\mathbf{0.88^{0.04}}$ & $\mathbf{0.96^{0.00}}$ & $\mathbf{0.99^{0.00}}$ \\
GRAF + OH + FP & $\mathbf{0.88^{0.03}}$ & $\mathbf{0.96^{0.00}}$ & $\mathbf{0.99^{0.00}}$ & $\mathbf{0.88^{0.03}}$ & $\mathbf{0.97^{0.00}}$ & $0.99^{0.00}$ & $\mathbf{0.88^{0.03}}$ & $\mathbf{0.96^{0.00}}$ & $\mathbf{0.99^{0.00}}$ \\
\hline
ZCP & $0.49^{0.05}$ & $0.63^{0.02}$ & $0.82^{0.01}$ & $0.49^{0.05}$ & $0.63^{0.02}$ & $0.83^{0.01}$ & $0.46^{0.06}$ & $0.61^{0.03}$ & $0.83^{0.01}$ \\
ZCP + OH & $0.53^{0.05}$ & $0.67^{0.03}$ & $0.82^{0.01}$ & $0.54^{0.06}$ & $0.67^{0.03}$ & $0.83^{0.01}$ & $0.51^{0.06}$ & $0.66^{0.03}$ & $0.82^{0.01}$ \\
ZCP + GRAF & $\mathbf{0.88^{0.04}}$ & $0.96^{0.00}$ & $\mathbf{0.99^{0.00}}$ & $\mathbf{0.88^{0.04}}$ & $\mathbf{0.96^{0.00}}$ & $\mathbf{0.99^{0.00}}$ & $\mathbf{0.87^{0.04}}$ & $0.96^{0.00}$ & $\mathbf{0.99^{0.00}}$ \\
ZCP + GRAF + OH & $\mathbf{0.88^{0.04}}$ & $\mathbf{0.96^{0.00}}$ & $\mathbf{0.99^{0.00}}$ & $0.88^{0.04}$ & $\mathbf{0.96^{0.00}}$ & $\mathbf{0.99^{0.00}}$ & $\mathbf{0.87^{0.04}}$ & $0.96^{0.00}$ & $\mathbf{0.99^{0.00}}$ \\
\end{tabular}
    \end{table}\begin{table}
    \small
    \addtolength{\tabcolsep}{-0.2em}
    \centering
    \caption{Results on the {\tt pixel3\_latency} task for various datasets. Average and standard deviation of Kendall tau over 50 independent runs. Bold values indicate the best results and those that are not statistically different from them. \label{ap:tab:pixlat}}
    \vskip 0.15in
    \begin{tabular}{r|ccc|ccc|ccc}
dataset & \multicolumn{3}{|c}{cifar10} & \multicolumn{3}{|c}{cifar100} & \multicolumn{3}{|c}{ImageNet16-120} \\
train\_size & 32 & 128 & 1024 & 32 & 128 & 1024 & 32 & 128 & 1024 \\
\hline
OH & $0.56^{0.07}$ & $0.72^{0.03}$ & $0.83^{0.00}$ & $0.56^{0.08}$ & $0.72^{0.03}$ & $0.83^{0.00}$ & $0.57^{0.08}$ & $0.72^{0.03}$ & $0.83^{0.00}$ \\
OH + FP & $0.76^{0.02}$ & $0.81^{0.01}$ & $0.86^{0.00}$ & $0.76^{0.02}$ & $0.81^{0.01}$ & $0.86^{0.00}$ & $0.78^{0.02}$ & $0.82^{0.01}$ & $0.86^{0.00}$ \\
GRAF & $\mathbf{0.80^{0.03}}$ & $\mathbf{0.85^{0.01}}$ & $0.87^{0.00}$ & $\mathbf{0.79^{0.03}}$ & $\mathbf{0.85^{0.01}}$ & $0.86^{0.00}$ & $\mathbf{0.81^{0.03}}$ & $\mathbf{0.85^{0.01}}$ & $0.87^{0.00}$ \\
GRAF + FP & $\mathbf{0.80^{0.02}}$ & $0.85^{0.01}$ & $0.87^{0.00}$ & $\mathbf{0.80^{0.02}}$ & $0.84^{0.01}$ & $0.86^{0.00}$ & $\mathbf{0.81^{0.02}}$ & $0.85^{0.01}$ & $0.87^{0.00}$ \\
GRAF + OH & $0.79^{0.03}$ & $\mathbf{0.85^{0.01}}$ & $0.87^{0.00}$ & $\mathbf{0.79^{0.03}}$ & $\mathbf{0.85^{0.01}}$ & $0.87^{0.00}$ & $\mathbf{0.80^{0.03}}$ & $\mathbf{0.85^{0.01}}$ & $0.87^{0.00}$ \\
GRAF + OH + FP & $\mathbf{0.80^{0.02}}$ & $0.85^{0.01}$ & $0.87^{0.00}$ & $\mathbf{0.80^{0.03}}$ & $0.84^{0.01}$ & $0.87^{0.00}$ & $\mathbf{0.81^{0.03}}$ & $0.85^{0.01}$ & $0.87^{0.00}$ \\
\hline
ZCP & $0.75^{0.02}$ & $0.80^{0.01}$ & $0.86^{0.00}$ & $0.75^{0.02}$ & $0.80^{0.01}$ & $0.85^{0.00}$ & $0.76^{0.02}$ & $0.80^{0.01}$ & $0.86^{0.00}$ \\
ZCP + OH & $0.75^{0.02}$ & $0.81^{0.01}$ & $0.86^{0.00}$ & $0.75^{0.02}$ & $0.81^{0.01}$ & $0.85^{0.00}$ & $0.77^{0.02}$ & $0.81^{0.01}$ & $0.86^{0.00}$ \\
ZCP + GRAF & $0.79^{0.02}$ & $0.84^{0.01}$ & $0.87^{0.00}$ & $\mathbf{0.79^{0.02}}$ & $0.84^{0.01}$ & $\mathbf{0.87^{0.00}}$ & $\mathbf{0.80^{0.03}}$ & $0.85^{0.01}$ & $0.87^{0.00}$ \\
ZCP + GRAF + OH & $0.79^{0.02}$ & $0.84^{0.01}$ & $\mathbf{0.87^{0.00}}$ & $\mathbf{0.79^{0.03}}$ & $0.84^{0.01}$ & $\mathbf{0.87^{0.00}}$ & $0.80^{0.03}$ & $0.85^{0.01}$ & $\mathbf{0.87^{0.00}}$ \\
\end{tabular}
    \end{table}\begin{table}
    \small
    \addtolength{\tabcolsep}{-0.2em}
    \centering
    \caption{Results on the {\tt edgetpu\_latency} task for various datasets. Average and standard deviation of Kendall tau over 50 independent runs. Bold values indicate the best results and those that are not statistically different from them. \label{ap:tab:tpulat}}
    \vskip 0.15in
    \begin{tabular}{r|ccc|ccc|ccc}
dataset & \multicolumn{3}{|c}{cifar10} & \multicolumn{3}{|c}{cifar100} & \multicolumn{3}{|c}{ImageNet16-120} \\
train\_size & 32 & 128 & 1024 & 32 & 128 & 1024 & 32 & 128 & 1024 \\
\hline
OH & $0.38^{0.09}$ & $0.56^{0.04}$ & $0.77^{0.01}$ & $0.37^{0.09}$ & $0.56^{0.04}$ & $0.76^{0.01}$ & $0.36^{0.09}$ & $0.55^{0.05}$ & $0.75^{0.02}$ \\
OH + FP & $0.36^{0.09}$ & $0.55^{0.04}$ & $\mathbf{0.78^{0.01}}$ & $0.36^{0.08}$ & $0.54^{0.04}$ & $\mathbf{0.77^{0.01}}$ & $0.35^{0.09}$ & $0.53^{0.05}$ & $\mathbf{0.76^{0.02}}$ \\
GRAF & $\mathbf{0.49^{0.11}}$ & $\mathbf{0.61^{0.04}}$ & $0.72^{0.01}$ & $\mathbf{0.48^{0.11}}$ & $0.60^{0.04}$ & $0.70^{0.01}$ & $\mathbf{0.45^{0.13}}$ & $\mathbf{0.58^{0.04}}$ & $0.68^{0.01}$ \\
GRAF + FP & $\mathbf{0.49^{0.11}}$ & $0.61^{0.04}$ & $0.72^{0.01}$ & $\mathbf{0.48^{0.11}}$ & $0.60^{0.04}$ & $0.70^{0.01}$ & $\mathbf{0.45^{0.13}}$ & $0.57^{0.04}$ & $0.68^{0.01}$ \\
GRAF + OH & $\mathbf{0.48^{0.11}}$ & $\mathbf{0.61^{0.04}}$ & $0.74^{0.01}$ & $\mathbf{0.48^{0.10}}$ & $\mathbf{0.60^{0.04}}$ & $0.72^{0.01}$ & $\mathbf{0.45^{0.13}}$ & $\mathbf{0.58^{0.04}}$ & $0.71^{0.01}$ \\
GRAF + OH + FP & $\mathbf{0.49^{0.10}}$ & $\mathbf{0.61^{0.04}}$ & $0.74^{0.01}$ & $\mathbf{0.48^{0.10}}$ & $\mathbf{0.60^{0.04}}$ & $0.72^{0.01}$ & $\mathbf{0.45^{0.13}}$ & $\mathbf{0.58^{0.04}}$ & $0.71^{0.01}$ \\
\hline
ZCP & $0.30^{0.07}$ & $0.37^{0.04}$ & $0.48^{0.01}$ & $0.30^{0.06}$ & $0.37^{0.03}$ & $0.47^{0.01}$ & $0.28^{0.08}$ & $0.34^{0.04}$ & $0.45^{0.02}$ \\
ZCP + OH & $0.35^{0.08}$ & $0.49^{0.04}$ & $0.69^{0.02}$ & $0.36^{0.07}$ & $0.48^{0.04}$ & $0.68^{0.02}$ & $0.33^{0.09}$ & $0.47^{0.04}$ & $0.66^{0.02}$ \\
ZCP + GRAF & $\mathbf{0.48^{0.10}}$ & $0.60^{0.04}$ & $0.71^{0.01}$ & $\mathbf{0.47^{0.09}}$ & $0.59^{0.03}$ & $0.70^{0.01}$ & $\mathbf{0.44^{0.13}}$ & $0.56^{0.04}$ & $0.67^{0.01}$ \\
ZCP + GRAF + OH & $\mathbf{0.49^{0.10}}$ & $0.60^{0.04}$ & $0.73^{0.01}$ & $\mathbf{0.48^{0.09}}$ & $0.59^{0.03}$ & $0.71^{0.01}$ & $\mathbf{0.44^{0.12}}$ & $0.57^{0.05}$ & $0.70^{0.01}$ \\
\end{tabular}
    \end{table}\begin{table}
    \small
    \addtolength{\tabcolsep}{-0.2em}
    \centering
    \caption{Results on the {\tt raspi4\_latency} task for various datasets. Average and standard deviation of Kendall tau over 50 independent runs. Bold values indicate the best results and those that are not statistically different from them. \label{ap:tab:raspilat}}
    \vskip 0.15in
    \begin{tabular}{r|ccc|ccc|ccc}
dataset & \multicolumn{3}{|c}{cifar10} & \multicolumn{3}{|c}{cifar100} & \multicolumn{3}{|c}{ImageNet16-120} \\
train\_size & 32 & 128 & 1024 & 32 & 128 & 1024 & 32 & 128 & 1024 \\
\hline
OH & $0.58^{0.08}$ & $0.73^{0.03}$ & $0.84^{0.00}$ & $0.56^{0.08}$ & $0.72^{0.03}$ & $0.83^{0.00}$ & $0.46^{0.09}$ & $0.61^{0.02}$ & $0.69^{0.00}$ \\
OH + FP & $0.80^{0.01}$ & $0.84^{0.01}$ & $0.87^{0.00}$ & $0.80^{0.02}$ & $0.84^{0.01}$ & $0.87^{0.00}$ & $0.65^{0.03}$ & $0.69^{0.01}$ & $0.72^{0.00}$ \\
GRAF & $0.80^{0.04}$ & $\mathbf{0.86^{0.01}}$ & $0.88^{0.00}$ & $\mathbf{0.81^{0.04}}$ & $\mathbf{0.86^{0.01}}$ & $0.88^{0.00}$ & $0.63^{0.04}$ & $\mathbf{0.70^{0.01}}$ & $0.73^{0.00}$ \\
GRAF + FP & $\mathbf{0.81^{0.02}}$ & $\mathbf{0.86^{0.01}}$ & $0.88^{0.00}$ & $\mathbf{0.81^{0.02}}$ & $\mathbf{0.86^{0.00}}$ & $0.88^{0.00}$ & $\mathbf{0.66^{0.03}}$ & $0.70^{0.01}$ & $0.73^{0.00}$ \\
GRAF + OH & $0.80^{0.03}$ & $\mathbf{0.86^{0.01}}$ & $\mathbf{0.88^{0.00}}$ & $0.80^{0.03}$ & $\mathbf{0.86^{0.01}}$ & $0.88^{0.00}$ & $0.63^{0.04}$ & $\mathbf{0.70^{0.01}}$ & $0.73^{0.00}$ \\
GRAF + OH + FP & $\mathbf{0.81^{0.03}}$ & $\mathbf{0.86^{0.01}}$ & $0.88^{0.00}$ & $\mathbf{0.81^{0.02}}$ & $\mathbf{0.86^{0.00}}$ & $0.88^{0.00}$ & $\mathbf{0.66^{0.02}}$ & $\mathbf{0.70^{0.01}}$ & $0.73^{0.00}$ \\
\hline
ZCP & $0.79^{0.02}$ & $0.84^{0.01}$ & $0.87^{0.00}$ & $0.79^{0.02}$ & $0.83^{0.01}$ & $0.87^{0.00}$ & $0.64^{0.03}$ & $0.68^{0.01}$ & $0.72^{0.00}$ \\
ZCP + OH & $0.79^{0.02}$ & $0.84^{0.01}$ & $0.87^{0.00}$ & $0.79^{0.02}$ & $0.84^{0.01}$ & $0.87^{0.00}$ & $0.64^{0.03}$ & $0.68^{0.01}$ & $0.72^{0.00}$ \\
ZCP + GRAF & $\mathbf{0.81^{0.02}}$ & $\mathbf{0.86^{0.01}}$ & $0.88^{0.00}$ & $\mathbf{0.81^{0.02}}$ & $0.86^{0.00}$ & $\mathbf{0.88^{0.00}}$ & $\mathbf{0.66^{0.03}}$ & $\mathbf{0.70^{0.01}}$ & $0.73^{0.00}$ \\
ZCP + GRAF + OH & $\mathbf{0.81^{0.02}}$ & $\mathbf{0.86^{0.01}}$ & $\mathbf{0.88^{0.00}}$ & $\mathbf{0.81^{0.02}}$ & $0.86^{0.00}$ & $\mathbf{0.88^{0.00}}$ & $\mathbf{0.66^{0.02}}$ & $\mathbf{0.70^{0.01}}$ & $\mathbf{0.73^{0.00}}$ \\
\end{tabular}
    \end{table}\begin{table}
    \small
    \addtolength{\tabcolsep}{-0.2em}
    \centering
    \caption{Results on the {\tt edgegpu\_latency} task for various datasets. Average and standard deviation of Kendall tau over 50 independent runs. Bold values indicate the best results and those that are not statistically different from them. \label{ap:tab:gpulat}}
    \vskip 0.15in
    \begin{tabular}{r|ccc|ccc|ccc}
dataset & \multicolumn{3}{|c}{cifar10} & \multicolumn{3}{|c}{cifar100} & \multicolumn{3}{|c}{ImageNet16-120} \\
train\_size & 32 & 128 & 1024 & 32 & 128 & 1024 & 32 & 128 & 1024 \\
\hline
OH & $0.48^{0.06}$ & $0.67^{0.04}$ & $0.84^{0.01}$ & $0.48^{0.06}$ & $0.67^{0.04}$ & $0.83^{0.01}$ & $0.47^{0.06}$ & $0.67^{0.04}$ & $0.84^{0.01}$ \\
OH + FP & $0.54^{0.05}$ & $0.68^{0.02}$ & $0.82^{0.01}$ & $0.54^{0.05}$ & $0.68^{0.02}$ & $0.82^{0.01}$ & $0.54^{0.04}$ & $0.68^{0.03}$ & $0.82^{0.01}$ \\
GRAF & $0.60^{0.03}$ & $0.71^{0.02}$ & $0.81^{0.01}$ & $0.60^{0.03}$ & $0.70^{0.02}$ & $0.81^{0.01}$ & $0.60^{0.03}$ & $0.71^{0.02}$ & $0.81^{0.01}$ \\
GRAF + FP & $0.60^{0.03}$ & $0.71^{0.02}$ & $0.81^{0.01}$ & $0.60^{0.03}$ & $0.70^{0.01}$ & $0.81^{0.01}$ & $0.60^{0.03}$ & $0.70^{0.02}$ & $0.81^{0.00}$ \\
GRAF + OH & $\mathbf{0.61^{0.03}}$ & $\mathbf{0.72^{0.02}}$ & $\mathbf{0.86^{0.01}}$ & $\mathbf{0.61^{0.03}}$ & $\mathbf{0.72^{0.02}}$ & $\mathbf{0.86^{0.01}}$ & $\mathbf{0.61^{0.03}}$ & $\mathbf{0.72^{0.02}}$ & $\mathbf{0.86^{0.01}}$ \\
GRAF + OH + FP & $\mathbf{0.61^{0.03}}$ & $\mathbf{0.72^{0.02}}$ & $0.86^{0.01}$ & $\mathbf{0.61^{0.03}}$ & $\mathbf{0.72^{0.02}}$ & $0.86^{0.01}$ & $\mathbf{0.61^{0.03}}$ & $\mathbf{0.72^{0.02}}$ & $0.86^{0.01}$ \\
\hline
ZCP & $0.50^{0.03}$ & $0.55^{0.01}$ & $0.62^{0.00}$ & $0.50^{0.03}$ & $0.55^{0.01}$ & $0.62^{0.00}$ & $0.49^{0.03}$ & $0.55^{0.01}$ & $0.61^{0.00}$ \\
ZCP + OH & $0.54^{0.04}$ & $0.65^{0.02}$ & $0.80^{0.01}$ & $0.55^{0.03}$ & $0.65^{0.03}$ & $0.80^{0.01}$ & $0.54^{0.03}$ & $0.65^{0.03}$ & $0.81^{0.01}$ \\
ZCP + GRAF & $0.60^{0.03}$ & $0.69^{0.02}$ & $0.81^{0.01}$ & $0.59^{0.03}$ & $0.69^{0.02}$ & $0.80^{0.01}$ & $0.59^{0.03}$ & $0.69^{0.02}$ & $0.81^{0.01}$ \\
ZCP + GRAF + OH & $0.60^{0.03}$ & $0.70^{0.02}$ & $0.85^{0.01}$ & $\mathbf{0.60^{0.03}}$ & $0.70^{0.02}$ & $0.85^{0.01}$ & $\mathbf{0.60^{0.03}}$ & $0.70^{0.02}$ & $0.85^{0.01}$ \\
\end{tabular}
    \end{table}\begin{table}
    \small
    \addtolength{\tabcolsep}{-0.2em}
    \centering
    \caption{Results on the {\tt edgegpu\_energy} task for various datasets. Average and standard deviation of Kendall tau over 50 independent runs. Bold values indicate the best results and those that are not statistically different from them. \label{ap:tab:edgegpuen}}
    \vskip 0.15in
    \begin{tabular}{r|ccc|ccc|ccc}
dataset & \multicolumn{3}{|c}{cifar10} & \multicolumn{3}{|c}{cifar100} & \multicolumn{3}{|c}{ImageNet16-120} \\
train\_size & 32 & 128 & 1024 & 32 & 128 & 1024 & 32 & 128 & 1024 \\
\hline
OH & $0.47^{0.06}$ & $0.66^{0.04}$ & $0.82^{0.01}$ & $0.47^{0.05}$ & $0.65^{0.04}$ & $0.82^{0.01}$ & $0.46^{0.06}$ & $0.66^{0.04}$ & $0.82^{0.01}$ \\
OH + FP & $0.57^{0.04}$ & $0.69^{0.02}$ & $0.82^{0.01}$ & $0.58^{0.04}$ & $0.69^{0.02}$ & $0.81^{0.01}$ & $0.56^{0.04}$ & $0.69^{0.02}$ & $0.81^{0.01}$ \\
GRAF & $0.61^{0.04}$ & $0.71^{0.02}$ & $0.81^{0.01}$ & $0.61^{0.04}$ & $0.70^{0.01}$ & $0.80^{0.01}$ & $0.61^{0.04}$ & $0.70^{0.02}$ & $0.81^{0.01}$ \\
GRAF + FP & $0.62^{0.03}$ & $0.71^{0.02}$ & $0.81^{0.01}$ & $0.62^{0.03}$ & $0.70^{0.01}$ & $0.80^{0.01}$ & $\mathbf{0.61^{0.03}}$ & $0.71^{0.02}$ & $0.81^{0.01}$ \\
GRAF + OH & $\mathbf{0.62^{0.04}}$ & $\mathbf{0.72^{0.02}}$ & $\mathbf{0.84^{0.01}}$ & $0.62^{0.04}$ & $\mathbf{0.72^{0.02}}$ & $\mathbf{0.84^{0.01}}$ & $\mathbf{0.62^{0.04}}$ & $\mathbf{0.72^{0.02}}$ & $\mathbf{0.85^{0.01}}$ \\
GRAF + OH + FP & $\mathbf{0.63^{0.03}}$ & $\mathbf{0.72^{0.02}}$ & $\mathbf{0.84^{0.01}}$ & $\mathbf{0.62^{0.03}}$ & $\mathbf{0.72^{0.02}}$ & $\mathbf{0.84^{0.01}}$ & $\mathbf{0.62^{0.03}}$ & $\mathbf{0.72^{0.02}}$ & $\mathbf{0.85^{0.01}}$ \\
\hline
ZCP & $0.54^{0.03}$ & $0.59^{0.01}$ & $0.65^{0.00}$ & $0.54^{0.03}$ & $0.59^{0.01}$ & $0.64^{0.00}$ & $0.52^{0.03}$ & $0.58^{0.01}$ & $0.64^{0.00}$ \\
ZCP + OH & $0.58^{0.03}$ & $0.66^{0.02}$ & $0.80^{0.01}$ & $0.58^{0.03}$ & $0.66^{0.02}$ & $0.79^{0.01}$ & $0.56^{0.03}$ & $0.66^{0.02}$ & $0.80^{0.01}$ \\
ZCP + GRAF & $0.61^{0.03}$ & $0.69^{0.02}$ & $0.80^{0.01}$ & $0.61^{0.03}$ & $0.69^{0.02}$ & $0.79^{0.01}$ & $\mathbf{0.61^{0.03}}$ & $0.69^{0.02}$ & $0.80^{0.01}$ \\
ZCP + GRAF + OH & $0.62^{0.03}$ & $0.70^{0.02}$ & $0.83^{0.01}$ & $\mathbf{0.62^{0.03}}$ & $0.70^{0.02}$ & $0.83^{0.01}$ & $\mathbf{0.61^{0.03}}$ & $0.70^{0.02}$ & $0.84^{0.01}$ \\
\end{tabular}
    \end{table}

==> hw_tables_old.tex <==
\begin{table}
\small
\addtolength{\tabcolsep}{-0.2em}
\centering
\caption{Results on the {\tt fpga\_energy} tasks for different datasets. Average and standard deviation of Kendall's tau over 50 independent runs.}
\label{ap:tab:fpgaen}
\vskip 0.15in\begin{tabular}{r|ccc|ccc|ccc}
dataset & \multicolumn{3}{|c}{cifar10} & \multicolumn{3}{|c}{cifar100} & \multicolumn{3}{|c}{ImageNet16-120} \\
train\_size & 32 & 128 & 1024 & 32 & 128 & 1024 & 32 & 128 & 1024 \\
\hline
Onehot & $0.55^{0.07}$ & $0.72^{0.04}$ & $0.85^{0.00}$ & $0.55^{0.07}$ & $0.72^{0.04}$ & $0.85^{0.00}$ & $0.58^{0.08}$ & $0.74^{0.03}$ & $0.89^{0.00}$ \\
GRAF & $0.81^{0.04}$ & \boldmath $0.95^{0.01}$ & \boldmath $1.00^{0.00}$ & $0.81^{0.04}$ & \boldmath $0.95^{0.01}$ & \boldmath $1.00^{0.00}$ & $0.85^{0.05}$ & $0.96^{0.01}$ & \boldmath $1.00^{0.00}$ \\
Onehot + F\&P & $0.83^{0.02}$ & $0.89^{0.01}$ & $0.97^{0.00}$ & $0.83^{0.02}$ & $0.89^{0.01}$ & $0.97^{0.00}$ & \boldmath $0.90^{0.02}$ & $0.95^{0.00}$ & $0.99^{0.00}$ \\
GRAF + Onehot & $0.81^{0.03}$ & $0.95^{0.01}$ & $1.00^{0.00}$ & $0.81^{0.03}$ & $0.95^{0.01}$ & $1.00^{0.00}$ & $0.85^{0.04}$ & $0.96^{0.01}$ & $1.00^{0.00}$ \\
GRAF + F\&P & $0.85^{0.02}$ & $0.94^{0.01}$ & $1.00^{0.00}$ & \boldmath $0.85^{0.02}$ & $0.94^{0.01}$ & $1.00^{0.00}$ & $0.89^{0.03}$ & \boldmath $0.96^{0.00}$ & $1.00^{0.00}$ \\
GRAF + Onehot + F\&P & \boldmath $0.85^{0.02}$ & $0.94^{0.01}$ & $1.00^{0.00}$ & $0.85^{0.02}$ & $0.94^{0.01}$ & $1.00^{0.00}$ & $0.88^{0.03}$ & $0.96^{0.00}$ & $1.00^{0.00}$ \\
\hline
ZCP + F\&P & $0.82^{0.02}$ & $0.88^{0.01}$ & $0.96^{0.00}$ & $0.82^{0.02}$ & $0.88^{0.01}$ & $0.96^{0.00}$ & $0.88^{0.02}$ & $0.94^{0.00}$ & $0.98^{0.00}$ \\
ZCP + Onehot + F\&P & $0.82^{0.02}$ & $0.88^{0.01}$ & $0.96^{0.00}$ & $0.82^{0.02}$ & $0.88^{0.01}$ & $0.96^{0.00}$ & $0.88^{0.02}$ & $0.94^{0.00}$ & $0.98^{0.00}$ \\
ZCP + GRAF + F\&P & $0.84^{0.03}$ & $0.93^{0.01}$ & $0.99^{0.00}$ & $0.85^{0.03}$ & $0.93^{0.01}$ & $0.99^{0.00}$ & $0.89^{0.03}$ & $0.96^{0.01}$ & $0.99^{0.00}$ \\
Everything & $0.84^{0.03}$ & $0.93^{0.01}$ & $0.99^{0.00}$ & $0.84^{0.03}$ & $0.93^{0.01}$ & $0.99^{0.00}$ & $0.89^{0.03}$ & $0.96^{0.01}$ & $1.00^{0.00}$ \\
\hline
\end{tabular}
\end{table}

\begin{table}
\small
\addtolength{\tabcolsep}{-0.2em}
\centering
\caption{Results on the {\tt fpga\_latency} tasks for different datasets. Average and standard deviation of Kendall's tau over 50 independent runs.}
\label{ap:tab:fpgalat}
\vskip 0.15in\begin{tabular}{r|ccc|ccc|ccc}
dataset & \multicolumn{3}{|c}{cifar10} & \multicolumn{3}{|c}{cifar100} & \multicolumn{3}{|c}{ImageNet16-120} \\
train\_size & 32 & 128 & 1024 & 32 & 128 & 1024 & 32 & 128 & 1024 \\
\hline
Onehot & $0.55^{0.07}$ & $0.72^{0.03}$ & $0.85^{0.00}$ & $0.55^{0.07}$ & $0.72^{0.03}$ & $0.85^{0.00}$ & $0.58^{0.08}$ & $0.74^{0.03}$ & $0.89^{0.00}$ \\
GRAF & $0.81^{0.04}$ & \boldmath $0.95^{0.01}$ & \boldmath $1.00^{0.00}$ & $0.81^{0.04}$ & \boldmath $0.95^{0.01}$ & \boldmath $1.00^{0.00}$ & $0.85^{0.05}$ & $0.96^{0.01}$ & \boldmath $1.00^{0.00}$ \\
Onehot + F\&P & $0.83^{0.02}$ & $0.89^{0.01}$ & $0.97^{0.00}$ & $0.83^{0.02}$ & $0.89^{0.01}$ & $0.97^{0.00}$ & \boldmath $0.90^{0.02}$ & $0.95^{0.00}$ & $0.99^{0.00}$ \\
GRAF + Onehot & $0.81^{0.04}$ & $0.95^{0.01}$ & $1.00^{0.00}$ & $0.81^{0.04}$ & $0.95^{0.01}$ & $1.00^{0.00}$ & $0.85^{0.04}$ & $0.96^{0.01}$ & $1.00^{0.00}$ \\
GRAF + F\&P & \boldmath $0.85^{0.02}$ & $0.94^{0.01}$ & $1.00^{0.00}$ & \boldmath $0.85^{0.02}$ & $0.94^{0.01}$ & $1.00^{0.00}$ & $0.89^{0.03}$ & \boldmath $0.96^{0.00}$ & $1.00^{0.00}$ \\
GRAF + Onehot + F\&P & $0.85^{0.02}$ & $0.94^{0.01}$ & $1.00^{0.00}$ & $0.85^{0.02}$ & $0.94^{0.01}$ & $1.00^{0.00}$ & $0.88^{0.03}$ & $0.96^{0.00}$ & $1.00^{0.00}$ \\
\hline
ZCP + F\&P & $0.82^{0.02}$ & $0.88^{0.01}$ & $0.96^{0.00}$ & $0.82^{0.02}$ & $0.88^{0.01}$ & $0.96^{0.00}$ & $0.88^{0.02}$ & $0.94^{0.00}$ & $0.98^{0.00}$ \\
ZCP + Onehot + F\&P & $0.82^{0.02}$ & $0.88^{0.01}$ & $0.96^{0.00}$ & $0.82^{0.02}$ & $0.88^{0.01}$ & $0.96^{0.00}$ & $0.88^{0.02}$ & $0.94^{0.00}$ & $0.98^{0.00}$ \\
ZCP + GRAF + F\&P & $0.84^{0.03}$ & $0.93^{0.01}$ & $0.99^{0.00}$ & $0.84^{0.03}$ & $0.93^{0.01}$ & $0.99^{0.00}$ & $0.89^{0.03}$ & $0.96^{0.01}$ & $1.00^{0.00}$ \\
Everything & $0.84^{0.03}$ & $0.93^{0.01}$ & $0.99^{0.00}$ & $0.84^{0.03}$ & $0.93^{0.01}$ & $0.99^{0.00}$ & $0.89^{0.03}$ & $0.96^{0.01}$ & $1.00^{0.00}$ \\
\hline
\end{tabular}
\end{table}

\begin{table}
\small
\addtolength{\tabcolsep}{-0.2em}
\centering
\caption{Results on the \texttt{eyeriss\_arithmetic\_intensity} tasks for different datasets. Average and standard deviation of Kendall's tau over 50 independent runs.}
\label{ap:tab:eyerissar}
\vskip 0.15in\begin{tabular}{r|ccc|ccc|ccc}
dataset & \multicolumn{3}{|c}{cifar10} & \multicolumn{3}{|c}{cifar100} & \multicolumn{3}{|c}{ImageNet16-120} \\
train\_size & 32 & 128 & 1024 & 32 & 128 & 1024 & 32 & 128 & 1024 \\
\hline
Onehot & $0.53^{0.08}$ & $0.73^{0.04}$ & $0.88^{0.01}$ & $0.53^{0.08}$ & $0.73^{0.04}$ & $0.88^{0.01}$ & $0.53^{0.08}$ & $0.73^{0.04}$ & $0.88^{0.01}$ \\
GRAF & $0.78^{0.05}$ & \boldmath $0.92^{0.01}$ & \boldmath $0.99^{0.00}$ & $0.78^{0.05}$ & \boldmath $0.92^{0.01}$ & \boldmath $0.99^{0.00}$ & $0.78^{0.05}$ & \boldmath $0.93^{0.01}$ & \boldmath $1.00^{0.00}$ \\
Onehot + F\&P & $0.65^{0.04}$ & $0.77^{0.02}$ & $0.94^{0.01}$ & $0.65^{0.04}$ & $0.77^{0.02}$ & $0.94^{0.01}$ & $0.64^{0.04}$ & $0.76^{0.03}$ & $0.92^{0.01}$ \\
GRAF + Onehot & $0.78^{0.05}$ & $0.92^{0.02}$ & $0.99^{0.00}$ & $0.78^{0.05}$ & $0.92^{0.02}$ & $0.99^{0.00}$ & $0.78^{0.05}$ & $0.93^{0.01}$ & $1.00^{0.00}$ \\
GRAF + F\&P & \boldmath $0.78^{0.05}$ & $0.91^{0.02}$ & $0.99^{0.00}$ & \boldmath $0.78^{0.05}$ & $0.91^{0.02}$ & $0.99^{0.00}$ & \boldmath $0.79^{0.05}$ & $0.93^{0.02}$ & $1.00^{0.00}$ \\
GRAF + Onehot + F\&P & $0.78^{0.05}$ & $0.91^{0.02}$ & $0.99^{0.00}$ & $0.78^{0.05}$ & $0.91^{0.02}$ & $0.99^{0.00}$ & $0.79^{0.05}$ & $0.93^{0.02}$ & $1.00^{0.00}$ \\
\hline
ZCP + F\&P & $0.61^{0.04}$ & $0.72^{0.02}$ & $0.88^{0.00}$ & $0.61^{0.04}$ & $0.72^{0.02}$ & $0.88^{0.01}$ & $0.62^{0.03}$ & $0.70^{0.01}$ & $0.85^{0.01}$ \\
ZCP + Onehot + F\&P & $0.63^{0.04}$ & $0.74^{0.02}$ & $0.89^{0.00}$ & $0.63^{0.04}$ & $0.74^{0.02}$ & $0.89^{0.00}$ & $0.64^{0.03}$ & $0.73^{0.02}$ & $0.88^{0.01}$ \\
ZCP + GRAF + F\&P & $0.75^{0.05}$ & $0.89^{0.02}$ & $0.99^{0.00}$ & $0.75^{0.05}$ & $0.89^{0.02}$ & $0.99^{0.00}$ & $0.78^{0.04}$ & $0.91^{0.02}$ & $0.99^{0.00}$ \\
Everything & $0.75^{0.05}$ & $0.89^{0.02}$ & $0.99^{0.00}$ & $0.75^{0.05}$ & $0.89^{0.02}$ & $0.99^{0.00}$ & $0.78^{0.04}$ & $0.91^{0.02}$ & $0.99^{0.00}$ \\
\hline
\end{tabular}
\end{table}

\begin{table}
\small
\addtolength{\tabcolsep}{-0.2em}
\centering
\caption{Results on the {\tt eyeriss\_energy} tasks for different datasets. Average and standard deviation of Kendall's tau over 50 independent runs.}
\label{ap:tab:eyerissen}
\vskip 0.15in\begin{tabular}{r|ccc|ccc|ccc}
dataset & \multicolumn{3}{|c}{cifar10} & \multicolumn{3}{|c}{cifar100} & \multicolumn{3}{|c}{ImageNet16-120} \\
train\_size & 32 & 128 & 1024 & 32 & 128 & 1024 & 32 & 128 & 1024 \\
\hline
Onehot & $0.48^{0.06}$ & $0.67^{0.05}$ & $0.84^{0.01}$ & $0.48^{0.06}$ & $0.67^{0.05}$ & $0.84^{0.01}$ & $0.48^{0.06}$ & $0.67^{0.05}$ & $0.84^{0.01}$ \\
GRAF & $0.87^{0.03}$ & $0.97^{0.00}$ & $1.00^{0.00}$ & $0.87^{0.04}$ & $0.97^{0.00}$ & $1.00^{0.00}$ & $0.87^{0.03}$ & $0.97^{0.00}$ & $1.00^{0.00}$ \\
Onehot + F\&P & $0.61^{0.04}$ & $0.76^{0.03}$ & $0.90^{0.01}$ & $0.62^{0.04}$ & $0.76^{0.03}$ & $0.90^{0.01}$ & $0.62^{0.04}$ & $0.76^{0.03}$ & $0.90^{0.01}$ \\
GRAF + Onehot & $0.87^{0.04}$ & $0.97^{0.00}$ & $1.00^{0.00}$ & $0.86^{0.04}$ & $0.97^{0.00}$ & $1.00^{0.00}$ & $0.87^{0.04}$ & $0.97^{0.00}$ & $1.00^{0.00}$ \\
GRAF + F\&P & $0.87^{0.04}$ & \boldmath $0.97^{0.00}$ & \boldmath $1.00^{0.00}$ & \boldmath $0.88^{0.04}$ & $0.97^{0.00}$ & $1.00^{0.00}$ & $0.87^{0.04}$ & $0.97^{0.00}$ & \boldmath $1.00^{0.00}$ \\
GRAF + Onehot + F\&P & $0.87^{0.03}$ & $0.97^{0.00}$ & $1.00^{0.00}$ & $0.87^{0.03}$ & $0.97^{0.00}$ & \boldmath $1.00^{0.00}$ & \boldmath $0.87^{0.04}$ & $0.97^{0.00}$ & $1.00^{0.00}$ \\
\hline
ZCP + F\&P & $0.56^{0.05}$ & $0.68^{0.02}$ & $0.84^{0.01}$ & $0.55^{0.05}$ & $0.68^{0.02}$ & $0.84^{0.01}$ & $0.53^{0.07}$ & $0.67^{0.02}$ & $0.85^{0.01}$ \\
ZCP + Onehot + F\&P & $0.59^{0.05}$ & $0.71^{0.03}$ & $0.84^{0.01}$ & $0.59^{0.05}$ & $0.71^{0.03}$ & $0.84^{0.01}$ & $0.57^{0.07}$ & $0.71^{0.03}$ & $0.84^{0.01}$ \\
ZCP + GRAF + F\&P & \boldmath $0.88^{0.04}$ & $0.97^{0.00}$ & $1.00^{0.00}$ & $0.88^{0.04}$ & \boldmath $0.97^{0.00}$ & $1.00^{0.00}$ & $0.87^{0.04}$ & \boldmath $0.97^{0.00}$ & $1.00^{0.00}$ \\
Everything & $0.87^{0.04}$ & $0.97^{0.00}$ & $1.00^{0.00}$ & $0.87^{0.04}$ & $0.97^{0.00}$ & $1.00^{0.00}$ & $0.87^{0.04}$ & $0.97^{0.00}$ & $1.00^{0.00}$ \\
\hline
\end{tabular}
\end{table}

\begin{table}
\small
\addtolength{\tabcolsep}{-0.2em}
\centering
\caption{Results on the {\tt eyeriss\_latency} tasks for different datasets. Average and standard deviation of Kendall's tau over 50 independent runs.}
\label{ap:tab:eyerisslat}
\vskip 0.15in\begin{tabular}{r|ccc|ccc|ccc}
dataset & \multicolumn{3}{|c}{cifar10} & \multicolumn{3}{|c}{cifar100} & \multicolumn{3}{|c}{ImageNet16-120} \\
train\_size & 32 & 128 & 1024 & 32 & 128 & 1024 & 32 & 128 & 1024 \\
\hline
Onehot & $0.49^{0.06}$ & $0.67^{0.04}$ & $0.84^{0.01}$ & $0.49^{0.06}$ & $0.68^{0.04}$ & $0.84^{0.01}$ & $0.49^{0.06}$ & $0.67^{0.04}$ & $0.84^{0.01}$ \\
GRAF & $0.88^{0.04}$ & $0.96^{0.00}$ & \boldmath $0.99^{0.00}$ & $0.88^{0.04}$ & $0.97^{0.00}$ & $0.99^{0.00}$ & $0.88^{0.03}$ & \boldmath $0.96^{0.00}$ & \boldmath $0.99^{0.00}$ \\
Onehot + F\&P & $0.56^{0.04}$ & $0.72^{0.03}$ & $0.90^{0.01}$ & $0.56^{0.04}$ & $0.72^{0.03}$ & $0.91^{0.01}$ & $0.56^{0.04}$ & $0.72^{0.03}$ & $0.90^{0.01}$ \\
GRAF + Onehot & $0.88^{0.04}$ & $0.96^{0.00}$ & $0.99^{0.00}$ & \boldmath $0.88^{0.04}$ & $0.97^{0.00}$ & $0.99^{0.00}$ & \boldmath $0.88^{0.04}$ & $0.96^{0.00}$ & $0.99^{0.00}$ \\
GRAF + F\&P & $0.88^{0.04}$ & \boldmath $0.96^{0.00}$ & $0.99^{0.00}$ & $0.88^{0.04}$ & \boldmath $0.97^{0.00}$ & \boldmath $0.99^{0.00}$ & $0.88^{0.04}$ & $0.96^{0.00}$ & $0.99^{0.00}$ \\
GRAF + Onehot + F\&P & \boldmath $0.88^{0.03}$ & $0.96^{0.00}$ & $0.99^{0.00}$ & $0.88^{0.03}$ & $0.97^{0.00}$ & $0.99^{0.00}$ & $0.88^{0.03}$ & $0.96^{0.00}$ & $0.99^{0.00}$ \\
\hline
ZCP + F\&P & $0.49^{0.05}$ & $0.63^{0.02}$ & $0.82^{0.01}$ & $0.49^{0.05}$ & $0.63^{0.02}$ & $0.83^{0.01}$ & $0.46^{0.06}$ & $0.61^{0.03}$ & $0.83^{0.01}$ \\
ZCP + Onehot + F\&P & $0.53^{0.05}$ & $0.67^{0.03}$ & $0.82^{0.01}$ & $0.54^{0.06}$ & $0.67^{0.03}$ & $0.83^{0.01}$ & $0.51^{0.06}$ & $0.66^{0.03}$ & $0.82^{0.01}$ \\
ZCP + GRAF + F\&P & $0.88^{0.04}$ & $0.96^{0.00}$ & $0.99^{0.00}$ & $0.88^{0.04}$ & $0.96^{0.00}$ & $0.99^{0.00}$ & $0.87^{0.04}$ & $0.96^{0.00}$ & $0.99^{0.00}$ \\
Everything & $0.88^{0.04}$ & $0.96^{0.00}$ & $0.99^{0.00}$ & $0.88^{0.04}$ & $0.96^{0.00}$ & $0.99^{0.00}$ & $0.87^{0.04}$ & $0.96^{0.00}$ & $0.99^{0.00}$ \\
\hline
\end{tabular}
\end{table}

\begin{table}
\small
\addtolength{\tabcolsep}{-0.2em}
\centering
\caption{Results on the {\tt pixel3\_latency} tasks for different datasets. Average and standard deviation of Kendall's tau over 50 independent runs.}
\label{ap:tab:pixlat}
\vskip 0.15in\begin{tabular}{r|ccc|ccc|ccc}
dataset & \multicolumn{3}{|c}{cifar10} & \multicolumn{3}{|c}{cifar100} & \multicolumn{3}{|c}{ImageNet16-120} \\
train\_size & 32 & 128 & 1024 & 32 & 128 & 1024 & 32 & 128 & 1024 \\
\hline
Onehot & $0.56^{0.07}$ & $0.72^{0.03}$ & $0.83^{0.00}$ & $0.56^{0.08}$ & $0.72^{0.03}$ & $0.83^{0.00}$ & $0.57^{0.08}$ & $0.72^{0.03}$ & $0.83^{0.00}$ \\
GRAF & $0.80^{0.03}$ & \boldmath $0.85^{0.01}$ & $0.87^{0.00}$ & $0.79^{0.03}$ & \boldmath $0.85^{0.01}$ & $0.86^{0.00}$ & $0.81^{0.03}$ & \boldmath $0.85^{0.01}$ & $0.87^{0.00}$ \\
Onehot + F\&P & $0.76^{0.02}$ & $0.81^{0.01}$ & $0.86^{0.00}$ & $0.76^{0.02}$ & $0.81^{0.01}$ & $0.86^{0.00}$ & $0.78^{0.02}$ & $0.82^{0.01}$ & $0.86^{0.00}$ \\
GRAF + Onehot & $0.79^{0.03}$ & $0.85^{0.01}$ & $0.87^{0.00}$ & $0.79^{0.03}$ & $0.85^{0.01}$ & $0.87^{0.00}$ & $0.80^{0.03}$ & $0.85^{0.01}$ & $0.87^{0.00}$ \\
GRAF + F\&P & \boldmath $0.80^{0.02}$ & $0.85^{0.01}$ & $0.87^{0.00}$ & \boldmath $0.80^{0.02}$ & $0.84^{0.01}$ & $0.86^{0.00}$ & \boldmath $0.81^{0.02}$ & $0.85^{0.01}$ & $0.87^{0.00}$ \\
GRAF + Onehot + F\&P & $0.80^{0.02}$ & $0.85^{0.01}$ & $0.87^{0.00}$ & $0.80^{0.03}$ & $0.84^{0.01}$ & $0.87^{0.00}$ & $0.81^{0.03}$ & $0.85^{0.01}$ & $0.87^{0.00}$ \\
\hline
ZCP + F\&P & $0.75^{0.02}$ & $0.80^{0.01}$ & $0.86^{0.00}$ & $0.75^{0.02}$ & $0.80^{0.01}$ & $0.85^{0.00}$ & $0.76^{0.02}$ & $0.80^{0.01}$ & $0.86^{0.00}$ \\
ZCP + Onehot + F\&P & $0.75^{0.02}$ & $0.81^{0.01}$ & $0.86^{0.00}$ & $0.75^{0.02}$ & $0.81^{0.01}$ & $0.85^{0.00}$ & $0.77^{0.02}$ & $0.81^{0.01}$ & $0.86^{0.00}$ \\
ZCP + GRAF + F\&P & $0.79^{0.02}$ & $0.84^{0.01}$ & $0.87^{0.00}$ & $0.79^{0.02}$ & $0.84^{0.01}$ & $0.87^{0.00}$ & $0.80^{0.03}$ & $0.85^{0.01}$ & $0.87^{0.00}$ \\
Everything & $0.79^{0.02}$ & $0.84^{0.01}$ & \boldmath $0.87^{0.00}$ & $0.79^{0.03}$ & $0.84^{0.01}$ & \boldmath $0.87^{0.00}$ & $0.80^{0.03}$ & $0.85^{0.01}$ & \boldmath $0.87^{0.00}$ \\
\hline
\end{tabular}
\end{table}
\begin{table}
\small
\addtolength{\tabcolsep}{-0.2em}
\centering
\caption{Results on the {\tt edgetpu\_latency} tasks for different datasets. Average and standard deviation of Kendall's tau over 50 independent runs.}
\label{ap:tab:tpulat}
\vskip 0.15in\begin{tabular}{r|ccc|ccc|ccc}
dataset & \multicolumn{3}{|c}{cifar10} & \multicolumn{3}{|c}{cifar100} & \multicolumn{3}{|c}{ImageNet16-120} \\
train\_size & 32 & 128 & 1024 & 32 & 128 & 1024 & 32 & 128 & 1024 \\
\hline
Onehot & $0.38^{0.09}$ & $0.56^{0.04}$ & $0.77^{0.01}$ & $0.37^{0.09}$ & $0.56^{0.04}$ & $0.76^{0.01}$ & $0.36^{0.09}$ & $0.55^{0.05}$ & $0.75^{0.02}$ \\
GRAF & $0.49^{0.11}$ & $0.61^{0.04}$ & $0.72^{0.01}$ & $0.48^{0.11}$ & $0.60^{0.04}$ & $0.70^{0.01}$ & $0.45^{0.13}$ & $0.58^{0.04}$ & $0.68^{0.01}$ \\
Onehot + F\&P & $0.36^{0.09}$ & $0.55^{0.04}$ & \boldmath $0.78^{0.01}$ & $0.36^{0.08}$ & $0.54^{0.04}$ & \boldmath $0.77^{0.01}$ & $0.35^{0.09}$ & $0.53^{0.05}$ & \boldmath $0.76^{0.02}$ \\
GRAF + Onehot & $0.48^{0.11}$ & \boldmath $0.61^{0.04}$ & $0.74^{0.01}$ & $0.48^{0.10}$ & $0.60^{0.04}$ & $0.72^{0.01}$ & $0.45^{0.13}$ & \boldmath $0.58^{0.04}$ & $0.71^{0.01}$ \\
GRAF + F\&P & $0.49^{0.11}$ & $0.61^{0.04}$ & $0.72^{0.01}$ & $0.48^{0.11}$ & $0.60^{0.04}$ & $0.70^{0.01}$ & $0.45^{0.13}$ & $0.57^{0.04}$ & $0.68^{0.01}$ \\
GRAF + Onehot + F\&P & \boldmath $0.49^{0.10}$ & $0.61^{0.04}$ & $0.74^{0.01}$ & \boldmath $0.48^{0.10}$ & \boldmath $0.60^{0.04}$ & $0.72^{0.01}$ & \boldmath $0.45^{0.13}$ & $0.58^{0.04}$ & $0.71^{0.01}$ \\
\hline
ZCP + F\&P & $0.30^{0.07}$ & $0.37^{0.04}$ & $0.48^{0.01}$ & $0.30^{0.06}$ & $0.37^{0.03}$ & $0.47^{0.01}$ & $0.28^{0.08}$ & $0.34^{0.04}$ & $0.45^{0.02}$ \\
ZCP + Onehot + F\&P & $0.35^{0.08}$ & $0.49^{0.04}$ & $0.69^{0.02}$ & $0.36^{0.07}$ & $0.48^{0.04}$ & $0.68^{0.02}$ & $0.33^{0.09}$ & $0.47^{0.04}$ & $0.66^{0.02}$ \\
ZCP + GRAF + F\&P & $0.48^{0.10}$ & $0.60^{0.04}$ & $0.71^{0.01}$ & $0.47^{0.09}$ & $0.59^{0.03}$ & $0.70^{0.01}$ & $0.44^{0.13}$ & $0.56^{0.04}$ & $0.67^{0.01}$ \\
Everything & $0.49^{0.10}$ & $0.60^{0.04}$ & $0.73^{0.01}$ & $0.48^{0.09}$ & $0.59^{0.03}$ & $0.71^{0.01}$ & $0.44^{0.12}$ & $0.57^{0.05}$ & $0.70^{0.01}$ \\
\hline
\end{tabular}
\end{table}

\begin{table}
\small
\addtolength{\tabcolsep}{-0.2em}
\centering
\caption{Results on the {\tt raspi4\_latency} tasks for different datasets. Average and standard deviation of Kendall's tau over 50 independent runs.}
\label{ap:tab:raspilat}
\vskip 0.15in\begin{tabular}{r|ccc|ccc|ccc}
dataset & \multicolumn{3}{|c}{cifar10} & \multicolumn{3}{|c}{cifar100} & \multicolumn{3}{|c}{ImageNet16-120} \\
train\_size & 32 & 128 & 1024 & 32 & 128 & 1024 & 32 & 128 & 1024 \\
\hline
Onehot & $0.58^{0.08}$ & $0.73^{0.03}$ & $0.84^{0.00}$ & $0.56^{0.08}$ & $0.72^{0.03}$ & $0.83^{0.00}$ & $0.46^{0.09}$ & $0.61^{0.02}$ & $0.69^{0.00}$ \\
GRAF & $0.80^{0.04}$ & \boldmath $0.86^{0.01}$ & $0.88^{0.00}$ & $0.81^{0.04}$ & $0.86^{0.01}$ & $0.88^{0.00}$ & $0.63^{0.04}$ & $0.70^{0.01}$ & $0.73^{0.00}$ \\
Onehot + F\&P & $0.80^{0.01}$ & $0.84^{0.01}$ & $0.87^{0.00}$ & $0.80^{0.02}$ & $0.84^{0.01}$ & $0.87^{0.00}$ & $0.65^{0.03}$ & $0.69^{0.01}$ & $0.72^{0.00}$ \\
GRAF + Onehot & $0.80^{0.03}$ & $0.86^{0.01}$ & $0.88^{0.00}$ & $0.80^{0.03}$ & $0.86^{0.01}$ & $0.88^{0.00}$ & $0.63^{0.04}$ & $0.70^{0.01}$ & $0.73^{0.00}$ \\
GRAF + F\&P & \boldmath $0.81^{0.02}$ & $0.86^{0.01}$ & $0.88^{0.00}$ & \boldmath $0.81^{0.02}$ & \boldmath $0.86^{0.00}$ & $0.88^{0.00}$ & \boldmath $0.66^{0.03}$ & $0.70^{0.01}$ & $0.73^{0.00}$ \\
GRAF + Onehot + F\&P & $0.81^{0.03}$ & $0.86^{0.01}$ & $0.88^{0.00}$ & $0.81^{0.02}$ & $0.86^{0.00}$ & $0.88^{0.00}$ & $0.66^{0.02}$ & \boldmath $0.70^{0.01}$ & $0.73^{0.00}$ \\
\hline
ZCP + F\&P & $0.79^{0.02}$ & $0.84^{0.01}$ & $0.87^{0.00}$ & $0.79^{0.02}$ & $0.83^{0.01}$ & $0.87^{0.00}$ & $0.64^{0.03}$ & $0.68^{0.01}$ & $0.72^{0.00}$ \\
ZCP + Onehot + F\&P & $0.79^{0.02}$ & $0.84^{0.01}$ & $0.87^{0.00}$ & $0.79^{0.02}$ & $0.84^{0.01}$ & $0.87^{0.00}$ & $0.64^{0.03}$ & $0.68^{0.01}$ & $0.72^{0.00}$ \\
ZCP + GRAF + F\&P & $0.81^{0.02}$ & $0.86^{0.01}$ & $0.88^{0.00}$ & $0.81^{0.02}$ & $0.86^{0.00}$ & $0.88^{0.00}$ & $0.66^{0.03}$ & $0.70^{0.01}$ & $0.73^{0.00}$ \\
Everything & $0.81^{0.02}$ & $0.86^{0.01}$ & \boldmath $0.88^{0.00}$ & $0.81^{0.02}$ & $0.86^{0.00}$ & \boldmath $0.88^{0.00}$ & $0.66^{0.02}$ & $0.70^{0.01}$ & \boldmath $0.73^{0.00}$ \\
\hline
\end{tabular}
\end{table}
\begin{table}
\small
\addtolength{\tabcolsep}{-0.2em}
\centering
\caption{Results on the {\tt edgegpu\_latency} tasks for different datasets. Average and standard deviation of Kendall's tau over 50 independent runs.}
\label{ap:tab:tpulat}
\vskip 0.15in\begin{tabular}{r|ccc|ccc|ccc}
dataset & \multicolumn{3}{|c}{cifar10} & \multicolumn{3}{|c}{cifar100} & \multicolumn{3}{|c}{ImageNet16-120} \\
train\_size & 32 & 128 & 1024 & 32 & 128 & 1024 & 32 & 128 & 1024 \\
\hline
Onehot & $0.48^{0.06}$ & $0.67^{0.04}$ & $0.84^{0.01}$ & $0.48^{0.06}$ & $0.67^{0.04}$ & $0.83^{0.01}$ & $0.47^{0.06}$ & $0.67^{0.04}$ & $0.84^{0.01}$ \\
GRAF & $0.60^{0.03}$ & $0.71^{0.02}$ & $0.81^{0.01}$ & $0.60^{0.03}$ & $0.70^{0.02}$ & $0.81^{0.01}$ & $0.60^{0.03}$ & $0.71^{0.02}$ & $0.81^{0.01}$ \\
Onehot + F\&P & $0.54^{0.05}$ & $0.68^{0.02}$ & $0.82^{0.01}$ & $0.54^{0.05}$ & $0.68^{0.02}$ & $0.82^{0.01}$ & $0.54^{0.04}$ & $0.68^{0.03}$ & $0.82^{0.01}$ \\
GRAF + Onehot & \boldmath $0.61^{0.03}$ & \boldmath $0.72^{0.02}$ & \boldmath $0.86^{0.01}$ & $0.61^{0.03}$ & \boldmath $0.72^{0.02}$ & \boldmath $0.86^{0.01}$ & \boldmath $0.61^{0.03}$ & \boldmath $0.72^{0.02}$ & \boldmath $0.86^{0.01}$ \\
GRAF + F\&P & $0.60^{0.03}$ & $0.71^{0.02}$ & $0.81^{0.01}$ & $0.60^{0.03}$ & $0.70^{0.01}$ & $0.81^{0.01}$ & $0.60^{0.03}$ & $0.70^{0.02}$ & $0.81^{0.00}$ \\
GRAF + Onehot + F\&P & $0.61^{0.03}$ & $0.72^{0.02}$ & $0.86^{0.01}$ & \boldmath $0.61^{0.03}$ & $0.72^{0.02}$ & $0.86^{0.01}$ & $0.61^{0.03}$ & $0.72^{0.02}$ & $0.86^{0.01}$ \\
\hline
ZCP + F\&P & $0.50^{0.03}$ & $0.55^{0.01}$ & $0.62^{0.00}$ & $0.50^{0.03}$ & $0.55^{0.01}$ & $0.62^{0.00}$ & $0.49^{0.03}$ & $0.55^{0.01}$ & $0.61^{0.00}$ \\
ZCP + Onehot + F\&P & $0.54^{0.04}$ & $0.65^{0.02}$ & $0.80^{0.01}$ & $0.55^{0.03}$ & $0.65^{0.03}$ & $0.80^{0.01}$ & $0.54^{0.03}$ & $0.65^{0.03}$ & $0.81^{0.01}$ \\
ZCP + GRAF + F\&P & $0.60^{0.03}$ & $0.69^{0.02}$ & $0.81^{0.01}$ & $0.59^{0.03}$ & $0.69^{0.02}$ & $0.80^{0.01}$ & $0.59^{0.03}$ & $0.69^{0.02}$ & $0.81^{0.01}$ \\
Everything & $0.60^{0.03}$ & $0.70^{0.02}$ & $0.85^{0.01}$ & $0.60^{0.03}$ & $0.70^{0.02}$ & $0.85^{0.01}$ & $0.60^{0.03}$ & $0.70^{0.02}$ & $0.85^{0.01}$ \\
\hline
\end{tabular}
\end{table}

\begin{table}
\small
\addtolength{\tabcolsep}{-0.2em}
\centering
\caption{Results on the {\tt edgegpu\_energy} tasks for different datasets. Average and standard deviation of Kendall's tau over 50 independent runs.}
\label{ap:tab:edgegpuen}
\vskip 0.15in\begin{tabular}{r|ccc|ccc|ccc}
dataset & \multicolumn{3}{|c}{cifar10} & \multicolumn{3}{|c}{cifar100} & \multicolumn{3}{|c}{ImageNet16-120} \\
train\_size & 32 & 128 & 1024 & 32 & 128 & 1024 & 32 & 128 & 1024 \\
\hline
Onehot & $0.47^{0.06}$ & $0.66^{0.04}$ & $0.82^{0.01}$ & $0.47^{0.05}$ & $0.65^{0.04}$ & $0.82^{0.01}$ & $0.46^{0.06}$ & $0.66^{0.04}$ & $0.82^{0.01}$ \\
GRAF & $0.61^{0.04}$ & $0.71^{0.02}$ & $0.81^{0.01}$ & $0.61^{0.04}$ & $0.70^{0.01}$ & $0.80^{0.01}$ & $0.61^{0.04}$ & $0.70^{0.02}$ & $0.81^{0.01}$ \\
Onehot + F\&P & $0.57^{0.04}$ & $0.69^{0.02}$ & $0.82^{0.01}$ & $0.58^{0.04}$ & $0.69^{0.02}$ & $0.81^{0.01}$ & $0.56^{0.04}$ & $0.69^{0.02}$ & $0.81^{0.01}$ \\
GRAF + Onehot & $0.62^{0.04}$ & \boldmath $0.72^{0.02}$ & $0.84^{0.01}$ & $0.62^{0.04}$ & \boldmath $0.72^{0.02}$ & \boldmath $0.84^{0.01}$ & $0.62^{0.04}$ & \boldmath $0.72^{0.02}$ & \boldmath $0.85^{0.01}$ \\
GRAF + F\&P & $0.62^{0.03}$ & $0.71^{0.02}$ & $0.81^{0.01}$ & $0.62^{0.03}$ & $0.70^{0.01}$ & $0.80^{0.01}$ & $0.61^{0.03}$ & $0.71^{0.02}$ & $0.81^{0.01}$ \\
GRAF + Onehot + F\&P & \boldmath $0.63^{0.03}$ & $0.72^{0.02}$ & \boldmath $0.84^{0.01}$ & \boldmath $0.62^{0.03}$ & $0.72^{0.02}$ & $0.84^{0.01}$ & \boldmath $0.62^{0.03}$ & $0.72^{0.02}$ & $0.85^{0.01}$ \\
\hline
ZCP + F\&P & $0.54^{0.03}$ & $0.59^{0.01}$ & $0.65^{0.00}$ & $0.54^{0.03}$ & $0.59^{0.01}$ & $0.64^{0.00}$ & $0.52^{0.03}$ & $0.58^{0.01}$ & $0.64^{0.00}$ \\
ZCP + Onehot + F\&P & $0.58^{0.03}$ & $0.66^{0.02}$ & $0.80^{0.01}$ & $0.58^{0.03}$ & $0.66^{0.02}$ & $0.79^{0.01}$ & $0.56^{0.03}$ & $0.66^{0.02}$ & $0.80^{0.01}$ \\
ZCP + GRAF + F\&P & $0.61^{0.03}$ & $0.69^{0.02}$ & $0.80^{0.01}$ & $0.61^{0.03}$ & $0.69^{0.02}$ & $0.79^{0.01}$ & $0.61^{0.03}$ & $0.69^{0.02}$ & $0.80^{0.01}$ \\
Everything & $0.62^{0.03}$ & $0.70^{0.02}$ & $0.83^{0.01}$ & $0.62^{0.03}$ & $0.70^{0.02}$ & $0.83^{0.01}$ & $0.61^{0.03}$ & $0.70^{0.02}$ & $0.84^{0.01}$ \\
\hline
\end{tabular}
\end{table}


==> important_feats_body.tex <==


\begin{table*}[h]
\caption{The ten most important features on NB201 (\texttt{cifar-10} and \texttt{ImageNet16-120} datasets) from ranking based on Shapley values computed from random forest trained on 1024 training samples with ZCP+GRAF.}
\label{featimp-nb201}
\vskip 0.1in
\small
\centering
\begin{tabular}{lrllr}
\hline
  \multicolumn{2}{c}{NB201 - \texttt{cifar-10}} && \multicolumn{2}{c}{NB201 - 
  \texttt{ImageNet16-120}} \\
Feature name &  Mean rank & $\quad$ &                   Feature name &  Mean rank \\
\hline
                         jacov &       0.00 &        &                          jacov &       0.00 \\
                          nwot &       1.12 &        & min path over [skip,C3x3,C1x1] &       2.30 \\
                         flops &       3.62 &        &                           nwot &       2.30 \\
                       synflow &       4.08 &        &                         params &       3.56 \\
min path over [skip,C3x3,C1x1] &       4.78 &        &                        synflow &       4.08 \\
                        params &       5.04 &        &                          flops &       4.30 \\
                       epe\_nas &       6.04 &        &      min path over [skip,C1x1] &       5.86 \\
                           zen &       6.36 &        &                            zen &       6.56 \\
     min path over [skip,C3x3] &      11.08 &        &                         fisher &       9.40 \\
            min path over skip &      11.88 &        &                      grad\_norm &      11.56 \\
\hline
\end{tabular}
\end{table*}




==> important_feats_body2.tex <==

\begin{table*}[h]
\caption{The ten most important features on TNB101-micro (\texttt{autoencoder} and \texttt{class\_scene} datasets) from ranking based on Shapley values computed from random forest trained on 1024 training samples with ZCP+GRAF.}
\label{featimp-tnb101}
\vskip 0.1in
\centering
\small
\begin{tabular}{lrllr}
\hline
\multicolumn{2}{c}{TNB101-micro - \texttt{autoencoder}} && \multicolumn{2}{c}{TNB101-micro - \texttt{class\_scene}} \\

             Feature name &  Mean rank & $\quad$ &                         Feature name &  Mean rank \\
\hline
       min path over skip &       0.00 &        &                               params &       0.28 \\
                    jacov &       1.00 &        &                                flops &       0.72 \\
                   fisher &       2.00 &        &              Average out deg. - C3x3 &       2.48 \\
min path over [skip,C3x3] &       5.50 &        &  Average out deg. - [zero,skip,C1x1] &       2.52 \\
                     snip &       5.58 &        &   Average in deg. - [zero,skip,C1x1] &       4.32 \\
min path over [skip,C1x1] &       5.64 &        &               Average in deg. - C3x3 &       4.68 \\
                grad\_norm &       6.64 &        &                       number of C3x3 &       6.00 \\
                      zen &       8.08 &        &                              synflow &       7.30 \\
                    grasp &       9.34 &        &      Input node degree - [zero,C1x1] &       9.34 \\
                  l2\_norm &       9.74 &        & Input node degree - [zero,C1x1,C3x3] &       9.42 \\
\hline
\end{tabular}
\end{table*}






==> redundant_features.tex <==

\begin{table}[hb]
\small
  \caption{Comparison of prediction with all GRAF features 
    and selected (linearly independent) GRAF features. Average of Kendall tau over 50 runs.}
  \label{ap:tab:redundancy}
  \centering
\begin{tabular}{l|rrr|rrr|rrr}
benchmark & \multicolumn{3}{c}{NB101} & \multicolumn{3}{c}{NB201} & \multicolumn{3}{c}{NB301} \\
train size &      32   &      128  &      1024 &      32   &      128  &      1024 &      32   &      128  &      1024 \\
features        &           &           &           &           &           &           &           &           &           \\
\hline
GRAF           &   $0.54^{0.08}$ & $0.63^{0.04}$ & $0.71^{0.01}$ & $0.63^{0.03}$ & $0.74^{0.01}$ & $0.83^{0.01}$ &  $0.38^{0.05}$ & $0.52^{0.03}$ & $0.61^{0.01}$ \\
sel. GRAF     &  $0.53^{0.08}$ &  $0.62^{0.04}$ &  $0.70^{0.01}$ &  $0.61^{0.04}$ &  $0.72^{0.02}$ &  $0.83^{0.00}$ &  $0.31^{0.06}$ &  $0.44^{0.02}$ &  $0.57^{0.01}$ \\
\hline
\end{tabular} 
\end{table}


==> tnb101_macro_tables.tex <==
\begin{table}[h]
    \small
    \addtolength{\tabcolsep}{-0.2em}
    \centering
    \caption{Results for various tasks of the TNB101-macro benchmark. Average and standard deviation of Kendall tau over 50 independent runs. Bold values indicate the best results and those that are not statistically different from them.}
    \vskip 0.15in
    \begin{tabular}{r|ccc|ccc|ccc}
dataset & \multicolumn{3}{|c}{autoencoder} & \multicolumn{3}{|c}{class\_object} & \multicolumn{3}{|c}{class\_scene} \\
train\_size & 32 & 128 & 1024 & 32 & 128 & 1024 & 32 & 128 & 1024 \\
\hline
OH & $0.38^{0.05}$ & $0.55^{0.03}$ & $0.71^{0.01}$ & $0.46^{0.05}$ & $0.58^{0.02}$ & $0.68^{0.01}$ & $0.56^{0.05}$ & $0.67^{0.02}$ & $0.76^{0.01}$ \\
OH + FP & $0.61^{0.04}$ & $0.70^{0.01}$ & $0.75^{0.00}$ & $0.60^{0.02}$ & $0.66^{0.01}$ & $0.70^{0.01}$ & $0.66^{0.03}$ & $0.73^{0.01}$ & $0.80^{0.00}$ \\
GRAF & $0.67^{0.03}$ & $\mathbf{0.73^{0.01}}$ & $0.77^{0.00}$ & $\mathbf{0.65^{0.03}}$ & $\mathbf{0.69^{0.01}}$ & $0.72^{0.00}$ & $\mathbf{0.69^{0.04}}$ & $\mathbf{0.77^{0.02}}$ & $\mathbf{0.83^{0.00}}$ \\
GRAF + FP & $\mathbf{0.68^{0.03}}$ & $\mathbf{0.74^{0.01}}$ & $0.77^{0.00}$ & $\mathbf{0.65^{0.02}}$ & $0.69^{0.01}$ & $0.72^{0.00}$ & $\mathbf{0.70^{0.02}}$ & $0.76^{0.01}$ & $0.82^{0.00}$ \\
GRAF + OH & $0.66^{0.03}$ & $0.73^{0.01}$ & $0.77^{0.00}$ & $0.64^{0.03}$ & $0.69^{0.01}$ & $\mathbf{0.72^{0.00}}$ & $0.68^{0.03}$ & $0.76^{0.01}$ & $0.83^{0.00}$ \\
GRAF + OH + FP & $0.67^{0.03}$ & $\mathbf{0.73^{0.01}}$ & $\mathbf{0.77^{0.00}}$ & $\mathbf{0.65^{0.02}}$ & $0.69^{0.01}$ & $\mathbf{0.72^{0.00}}$ & $0.69^{0.03}$ & $0.75^{0.01}$ & $0.82^{0.00}$ \\
\hline
ZCP & $0.59^{0.04}$ & $0.68^{0.01}$ & $0.73^{0.00}$ & $0.65^{0.02}$ & $0.68^{0.01}$ & $0.71^{0.00}$ & $0.70^{0.02}$ & $0.74^{0.01}$ & $0.79^{0.00}$ \\
ZCP + OH & $0.59^{0.04}$ & $0.69^{0.01}$ & $0.74^{0.01}$ & $0.65^{0.02}$ & $0.69^{0.01}$ & $0.71^{0.00}$ & $0.70^{0.02}$ & $0.75^{0.01}$ & $0.81^{0.00}$ \\
ZCP + GRAF & $0.65^{0.03}$ & $0.73^{0.01}$ & $0.77^{0.00}$ & $\mathbf{0.66^{0.02}}$ & $0.69^{0.01}$ & $0.72^{0.00}$ & $\mathbf{0.71^{0.02}}$ & $0.75^{0.01}$ & $0.81^{0.00}$ \\
ZCP + GRAF + OH & $0.65^{0.03}$ & $0.73^{0.01}$ & $0.77^{0.00}$ & $\mathbf{0.66^{0.02}}$ & $\mathbf{0.69^{0.01}}$ & $\mathbf{0.72^{0.00}}$ & $\mathbf{0.70^{0.02}}$ & $0.76^{0.01}$ & $0.82^{0.00}$ \\
\end{tabular}
    \end{table}\begin{table}
    \small
    \addtolength{\tabcolsep}{-0.2em}
    \centering
    \caption{Results for various tasks of the TNB101-macro benchmark. Average and standard deviation of Kendall tau over 50 independent runs. Bold values indicate the best results and those that are not statistically different from them.}
    \vskip 0.15in
    \begin{tabular}{r|ccc|ccc|ccc}
dataset & \multicolumn{3}{|c}{jigsaw} & \multicolumn{3}{|c}{normal} & \multicolumn{3}{|c}{room\_layout} \\
train\_size & 32 & 128 & 1024 & 32 & 128 & 1024 & 32 & 128 & 1024 \\
\hline
OH & $0.59^{0.04}$ & $0.64^{0.01}$ & $0.66^{0.00}$ & $0.40^{0.05}$ & $0.49^{0.04}$ & $0.55^{0.01}$ & $0.47^{0.06}$ & $0.54^{0.03}$ & $0.60^{0.01}$ \\
OH + FP & $0.58^{0.04}$ & $\mathbf{0.65^{0.01}}$ & $0.67^{0.00}$ & $0.55^{0.03}$ & $0.57^{0.03}$ & $0.60^{0.01}$ & $0.46^{0.06}$ & $0.55^{0.03}$ & $0.61^{0.01}$ \\
GRAF & $0.60^{0.03}$ & $\mathbf{0.65^{0.01}}$ & $0.67^{0.00}$ & $0.54^{0.03}$ & $0.57^{0.02}$ & $0.60^{0.01}$ & $\mathbf{0.51^{0.04}}$ & $\mathbf{0.57^{0.02}}$ & $0.62^{0.01}$ \\
GRAF + FP & $0.60^{0.03}$ & $\mathbf{0.65^{0.01}}$ & $0.67^{0.00}$ & $\mathbf{0.56^{0.03}}$ & $\mathbf{0.58^{0.03}}$ & $0.60^{0.01}$ & $0.50^{0.05}$ & $\mathbf{0.57^{0.02}}$ & $0.62^{0.01}$ \\
GRAF + OH & $\mathbf{0.61^{0.03}}$ & $\mathbf{0.65^{0.01}}$ & $0.67^{0.00}$ & $0.53^{0.03}$ & $0.57^{0.03}$ & $0.60^{0.01}$ & $\mathbf{0.51^{0.04}}$ & $\mathbf{0.57^{0.03}}$ & $0.63^{0.01}$ \\
GRAF + OH + FP & $\mathbf{0.61^{0.03}}$ & $\mathbf{0.65^{0.01}}$ & $0.68^{0.00}$ & $\mathbf{0.56^{0.03}}$ & $\mathbf{0.58^{0.03}}$ & $0.60^{0.01}$ & $\mathbf{0.50^{0.04}}$ & $\mathbf{0.57^{0.03}}$ & $0.63^{0.01}$ \\
\hline
ZCP & $0.49^{0.04}$ & $0.56^{0.01}$ & $0.62^{0.01}$ & $0.55^{0.03}$ & $0.57^{0.05}$ & $0.60^{0.01}$ & $0.39^{0.05}$ & $0.48^{0.02}$ & $0.56^{0.01}$ \\
ZCP + OH & $0.57^{0.04}$ & $\mathbf{0.65^{0.01}}$ & $0.67^{0.00}$ & $0.55^{0.03}$ & $0.58^{0.04}$ & $0.60^{0.01}$ & $0.45^{0.05}$ & $\mathbf{0.56^{0.02}}$ & $0.63^{0.01}$ \\
ZCP + GRAF & $0.59^{0.04}$ & $\mathbf{0.65^{0.01}}$ & $0.68^{0.00}$ & $\mathbf{0.56^{0.03}}$ & $\mathbf{0.58^{0.04}}$ & $0.61^{0.01}$ & $0.48^{0.05}$ & $0.56^{0.02}$ & $0.63^{0.01}$ \\
ZCP + GRAF + OH & $\mathbf{0.61^{0.03}}$ & $\mathbf{0.65^{0.01}}$ & $\mathbf{0.68^{0.00}}$ & $\mathbf{0.56^{0.02}}$ & $\mathbf{0.58^{0.05}}$ & $\mathbf{0.61^{0.01}}$ & $0.49^{0.05}$ & $\mathbf{0.57^{0.02}}$ & $\mathbf{0.63^{0.01}}$ \\
\end{tabular}
    \end{table}\begin{table}[h]
    \small
    \addtolength{\tabcolsep}{-0.2em}
    \centering
    \caption{Results for various tasks of the TNB101-macro benchmark. Average and standard deviation of Kendall tau over 50 independent runs. Bold values indicate the best results and those that are not statistically different from them.\label{acc-tnbmacro-table}}
    \vskip 0.15in
    \begin{tabular}{r|ccc}
dataset & \multicolumn{3}{|c}{segmentsemantic} \\
train\_size & 32 & 128 & 1024 \\
\hline
OH & $0.65^{0.04}$ & $0.74^{0.01}$ & $0.80^{0.00}$ \\
OH + FP & $0.62^{0.06}$ & $0.73^{0.02}$ & $0.81^{0.00}$ \\
GRAF & $\mathbf{0.69^{0.02}}$ & $\mathbf{0.76^{0.01}}$ & $0.82^{0.00}$ \\
GRAF + FP & $0.68^{0.04}$ & $0.76^{0.01}$ & $0.82^{0.00}$ \\
GRAF + OH & $\mathbf{0.69^{0.02}}$ & $\mathbf{0.76^{0.01}}$ & $\mathbf{0.82^{0.00}}$ \\
GRAF + OH + FP & $\mathbf{0.68^{0.04}}$ & $0.76^{0.01}$ & $\mathbf{0.82^{0.00}}$ \\
\hline
ZCP & $0.55^{0.03}$ & $0.66^{0.01}$ & $0.76^{0.01}$ \\
ZCP + OH & $0.60^{0.04}$ & $0.72^{0.01}$ & $0.80^{0.00}$ \\
ZCP + GRAF & $0.65^{0.04}$ & $0.74^{0.01}$ & $0.81^{0.00}$ \\
ZCP + GRAF + OH & $0.66^{0.04}$ & $0.74^{0.01}$ & $0.81^{0.00}$ \\
\end{tabular}
    \end{table}%

==> tnb101_micro_tables.tex <==
\begin{table}[h]
    \small
    \addtolength{\tabcolsep}{-0.2em}
    \centering
    \caption{Results for various tasks of the TNB101-micro benchmark. Average and standard deviation of Kendall tau over 50 independent runs. Bold values indicate the best results and those that are not statistically different from them.}
    \vskip 0.15in
    \begin{tabular}{r|ccc|ccc|ccc}
dataset & \multicolumn{3}{|c}{autoencoder} & \multicolumn{3}{|c}{class\_object} & \multicolumn{3}{|c}{class\_scene} \\
train\_size & 32 & 128 & 1024 & 32 & 128 & 1024 & 32 & 128 & 1024 \\
\hline
OH & $0.42^{0.06}$ & $0.55^{0.02}$ & $0.60^{0.01}$ & $0.23^{0.06}$ & $0.41^{0.04}$ & $0.61^{0.01}$ & $0.29^{0.06}$ & $0.51^{0.04}$ & $0.72^{0.01}$ \\
OH + FP & $0.39^{0.07}$ & $0.54^{0.03}$ & $0.60^{0.01}$ & $0.46^{0.05}$ & $0.55^{0.02}$ & $0.62^{0.01}$ & $0.51^{0.03}$ & $0.61^{0.02}$ & $0.72^{0.01}$ \\
GRAF & $\mathbf{0.56^{0.03}}$ & $\mathbf{0.59^{0.01}}$ & $0.63^{0.01}$ & $\mathbf{0.53^{0.03}}$ & $\mathbf{0.60^{0.01}}$ & $0.64^{0.01}$ & $\mathbf{0.58^{0.03}}$ & $0.67^{0.01}$ & $0.75^{0.01}$ \\
GRAF + FP & $\mathbf{0.56^{0.03}}$ & $\mathbf{0.59^{0.01}}$ & $0.63^{0.01}$ & $\mathbf{0.53^{0.04}}$ & $\mathbf{0.60^{0.01}}$ & $0.64^{0.01}$ & $\mathbf{0.58^{0.03}}$ & $0.67^{0.01}$ & $0.75^{0.01}$ \\
GRAF + OH & $\mathbf{0.55^{0.03}}$ & $\mathbf{0.59^{0.01}}$ & $0.63^{0.01}$ & $\mathbf{0.53^{0.03}}$ & $0.60^{0.01}$ & $0.64^{0.01}$ & $\mathbf{0.58^{0.03}}$ & $0.67^{0.02}$ & $0.75^{0.01}$ \\
GRAF + OH + FP & $\mathbf{0.55^{0.03}}$ & $\mathbf{0.59^{0.01}}$ & $0.63^{0.01}$ & $0.52^{0.04}$ & $0.60^{0.01}$ & $0.64^{0.01}$ & $\mathbf{0.57^{0.03}}$ & $0.67^{0.02}$ & $0.75^{0.01}$ \\
\hline
ZCP & $0.46^{0.04}$ & $0.52^{0.02}$ & $0.56^{0.01}$ & $0.41^{0.05}$ & $0.53^{0.01}$ & $0.60^{0.01}$ & $0.52^{0.03}$ & $0.60^{0.02}$ & $0.71^{0.01}$ \\
ZCP + OH & $0.48^{0.04}$ & $0.55^{0.02}$ & $0.60^{0.01}$ & $0.43^{0.06}$ & $0.55^{0.02}$ & $0.62^{0.01}$ & $0.53^{0.03}$ & $0.64^{0.02}$ & $0.74^{0.01}$ \\
ZCP + GRAF & $\mathbf{0.55^{0.03}}$ & $\mathbf{0.60^{0.01}}$ & $\mathbf{0.63^{0.01}}$ & $0.50^{0.05}$ & $0.60^{0.02}$ & $\mathbf{0.65^{0.01}}$ & $\mathbf{0.58^{0.04}}$ & $\mathbf{0.69^{0.02}}$ & $0.77^{0.01}$ \\
ZCP + GRAF + OH & $\mathbf{0.55^{0.03}}$ & $0.60^{0.01}$ & $\mathbf{0.63^{0.01}}$ & $0.51^{0.05}$ & $0.60^{0.02}$ & $\mathbf{0.65^{0.01}}$ & $\mathbf{0.59^{0.04}}$ & $\mathbf{0.69^{0.02}}$ & $\mathbf{0.77^{0.01}}$ \\
\hline
OH + PE & $0.47^{0.06}$ & $0.54^{0.02}$ & $0.60^{0.01}$ & $0.23^{0.06}$ & $0.35^{0.02}$ & $0.60^{0.01}$ & $0.30^{0.04}$ & $0.45^{0.02}$ & $0.72^{0.01}$ \\
OH + FP + PE & $0.45^{0.07}$ & $0.56^{0.02}$ & $0.61^{0.01}$ & $0.45^{0.06}$ & $0.55^{0.02}$ & $0.62^{0.01}$ & $0.51^{0.04}$ & $0.60^{0.02}$ & $0.73^{0.01}$ \\
GRAF + PE & $\mathbf{0.55^{0.03}}$ & $\mathbf{0.59^{0.01}}$ & $0.62^{0.01}$ & $\mathbf{0.53^{0.04}}$ & $\mathbf{0.60^{0.01}}$ & $0.64^{0.01}$ & $\mathbf{0.57^{0.03}}$ & $0.67^{0.02}$ & $0.75^{0.01}$ \\
GRAF + FP + PE & $\mathbf{0.55^{0.03}}$ & $\mathbf{0.59^{0.01}}$ & $0.63^{0.01}$ & $\mathbf{0.53^{0.04}}$ & $\mathbf{0.60^{0.01}}$ & $0.64^{0.01}$ & $\mathbf{0.58^{0.03}}$ & $0.67^{0.02}$ & $0.75^{0.01}$ \\
GRAF + OH + PE & $\mathbf{0.55^{0.03}}$ & $\mathbf{0.59^{0.01}}$ & $0.62^{0.01}$ & $\mathbf{0.52^{0.04}}$ & $0.60^{0.01}$ & $0.64^{0.01}$ & $0.57^{0.04}$ & $0.67^{0.02}$ & $0.75^{0.01}$ \\
GRAF + OH + FP + PE & $\mathbf{0.55^{0.03}}$ & $\mathbf{0.59^{0.01}}$ & $0.62^{0.01}$ & $\mathbf{0.53^{0.04}}$ & $0.60^{0.01}$ & $0.64^{0.01}$ & $\mathbf{0.57^{0.04}}$ & $0.67^{0.02}$ & $0.76^{0.01}$ \\
\hline
ZCP + PE & $0.50^{0.04}$ & $0.57^{0.02}$ & $0.61^{0.01}$ & $0.43^{0.05}$ & $0.55^{0.02}$ & $0.62^{0.01}$ & $0.53^{0.03}$ & $0.63^{0.02}$ & $0.73^{0.01}$ \\
ZCP + OH + PE & $0.49^{0.05}$ & $0.57^{0.02}$ & $0.61^{0.01}$ & $0.43^{0.06}$ & $0.55^{0.02}$ & $0.63^{0.01}$ & $0.53^{0.03}$ & $0.64^{0.02}$ & $0.74^{0.01}$ \\
ZCP + GRAF + PE & $\mathbf{0.55^{0.03}}$ & $\mathbf{0.59^{0.01}}$ & $\mathbf{0.63^{0.01}}$ & $0.50^{0.05}$ & $\mathbf{0.60^{0.02}}$ & $\mathbf{0.65^{0.01}}$ & $\mathbf{0.58^{0.04}}$ & $\mathbf{0.69^{0.02}}$ & $0.77^{0.01}$ \\
ZCP + GRAF + OH + PE & $\mathbf{0.55^{0.03}}$ & $\mathbf{0.59^{0.01}}$ & $0.63^{0.01}$ & $0.50^{0.05}$ & $\mathbf{0.60^{0.02}}$ & $\mathbf{0.65^{0.01}}$ & $\mathbf{0.58^{0.04}}$ & $\mathbf{0.69^{0.02}}$ & $\mathbf{0.77^{0.01}}$ \\
\end{tabular}
    \end{table}\begin{table}[h]
    \small
    \addtolength{\tabcolsep}{-0.2em}
    \centering
    \caption{Results for various tasks of the TNB101-micro benchmark. Average and standard deviation of Kendall tau over 50 independent runs. Bold values indicate the best results and those that are not statistically different from them.}
    \vskip 0.15in
    \begin{tabular}{r|ccc|ccc|ccc}
dataset & \multicolumn{3}{|c}{jigsaw} & \multicolumn{3}{|c}{normal} & \multicolumn{3}{|c}{room\_layout} \\
train\_size & 32 & 128 & 1024 & 32 & 128 & 1024 & 32 & 128 & 1024 \\
\hline
OH & $0.22^{0.05}$ & $0.35^{0.03}$ & $0.53^{0.01}$ & $0.31^{0.06}$ & $0.48^{0.03}$ & $0.55^{0.01}$ & $0.20^{0.07}$ & $0.36^{0.04}$ & $0.67^{0.04}$ \\
OH + FP & $0.41^{0.04}$ & $0.49^{0.01}$ & $0.56^{0.01}$ & $0.46^{0.05}$ & $0.53^{0.03}$ & $0.60^{0.01}$ & $0.59^{0.05}$ & $0.68^{0.02}$ & $0.77^{0.01}$ \\
GRAF & $\mathbf{0.47^{0.03}}$ & $\mathbf{0.53^{0.02}}$ & $0.57^{0.01}$ & $0.50^{0.04}$ & $0.54^{0.02}$ & $0.60^{0.01}$ & $\mathbf{0.67^{0.03}}$ & $0.74^{0.01}$ & $0.78^{0.01}$ \\
GRAF + FP & $\mathbf{0.47^{0.03}}$ & $\mathbf{0.53^{0.02}}$ & $0.57^{0.01}$ & $0.50^{0.04}$ & $0.55^{0.02}$ & $0.61^{0.01}$ & $\mathbf{0.67^{0.03}}$ & $0.74^{0.01}$ & $0.79^{0.01}$ \\
GRAF + OH & $\mathbf{0.47^{0.03}}$ & $\mathbf{0.53^{0.01}}$ & $0.58^{0.01}$ & $0.49^{0.04}$ & $0.55^{0.02}$ & $0.60^{0.01}$ & $\mathbf{0.66^{0.04}}$ & $0.74^{0.01}$ & $0.79^{0.01}$ \\
GRAF + OH + FP & $\mathbf{0.47^{0.04}}$ & $\mathbf{0.54^{0.01}}$ & $0.58^{0.01}$ & $0.50^{0.04}$ & $\mathbf{0.55^{0.02}}$ & $0.61^{0.01}$ & $\mathbf{0.67^{0.03}}$ & $0.74^{0.01}$ & $0.79^{0.01}$ \\
\hline
ZCP & $0.38^{0.04}$ & $0.46^{0.02}$ & $0.54^{0.01}$ & $0.48^{0.04}$ & $0.53^{0.02}$ & $0.59^{0.01}$ & $0.61^{0.06}$ & $0.72^{0.01}$ & $0.78^{0.01}$ \\
ZCP + OH & $0.40^{0.04}$ & $0.48^{0.02}$ & $0.56^{0.01}$ & $0.48^{0.04}$ & $0.54^{0.03}$ & $0.60^{0.01}$ & $0.61^{0.06}$ & $0.72^{0.01}$ & $0.78^{0.01}$ \\
ZCP + GRAF & $\mathbf{0.45^{0.03}}$ & $0.52^{0.02}$ & $\mathbf{0.59^{0.01}}$ & $\mathbf{0.51^{0.04}}$ & $\mathbf{0.55^{0.02}}$ & $0.62^{0.01}$ & $\mathbf{0.66^{0.05}}$ & $\mathbf{0.75^{0.02}}$ & $\mathbf{0.79^{0.01}}$ \\
ZCP + GRAF + OH & $\mathbf{0.46^{0.03}}$ & $0.52^{0.02}$ & $\mathbf{0.59^{0.01}}$ & $\mathbf{0.51^{0.03}}$ & $\mathbf{0.55^{0.02}}$ & $\mathbf{0.62^{0.01}}$ & $\mathbf{0.67^{0.04}}$ & $\mathbf{0.75^{0.02}}$ & $\mathbf{0.80^{0.01}}$ \\
\hline
OH + PE & $0.20^{0.05}$ & $0.31^{0.02}$ & $0.49^{0.02}$ & $0.31^{0.05}$ & $0.44^{0.03}$ & $0.55^{0.01}$ & $0.23^{0.08}$ & $0.35^{0.03}$ & $0.65^{0.05}$ \\
OH + FP + PE & $0.38^{0.04}$ & $0.46^{0.02}$ & $0.55^{0.01}$ & $0.47^{0.04}$ & $0.52^{0.02}$ & $0.59^{0.01}$ & $0.60^{0.05}$ & $0.70^{0.02}$ & $0.78^{0.01}$ \\
GRAF + PE & $\mathbf{0.46^{0.03}}$ & $0.52^{0.02}$ & $0.58^{0.01}$ & $0.50^{0.04}$ & $0.54^{0.02}$ & $0.60^{0.01}$ & $\mathbf{0.66^{0.04}}$ & $0.74^{0.01}$ & $0.79^{0.01}$ \\
GRAF + FP + PE & $\mathbf{0.46^{0.04}}$ & $0.53^{0.02}$ & $0.58^{0.01}$ & $0.50^{0.04}$ & $0.55^{0.02}$ & $0.61^{0.01}$ & $\mathbf{0.67^{0.03}}$ & $0.74^{0.01}$ & $0.79^{0.01}$ \\
GRAF + OH + PE & $0.46^{0.03}$ & $0.52^{0.02}$ & $0.58^{0.01}$ & $0.50^{0.04}$ & $0.55^{0.02}$ & $0.60^{0.01}$ & $\mathbf{0.66^{0.04}}$ & $0.74^{0.01}$ & $0.79^{0.01}$ \\
GRAF + OH + FP + PE & $0.46^{0.03}$ & $0.52^{0.02}$ & $0.58^{0.01}$ & $0.50^{0.04}$ & $0.55^{0.02}$ & $0.61^{0.01}$ & $\mathbf{0.67^{0.03}}$ & $0.74^{0.01}$ & $0.79^{0.01}$ \\
\hline
ZCP + PE & $0.39^{0.04}$ & $0.47^{0.02}$ & $0.55^{0.01}$ & $0.48^{0.03}$ & $0.53^{0.02}$ & $0.60^{0.01}$ & $0.62^{0.06}$ & $0.72^{0.01}$ & $0.78^{0.01}$ \\
ZCP + OH + PE & $0.39^{0.04}$ & $0.47^{0.02}$ & $0.56^{0.01}$ & $0.48^{0.03}$ & $0.54^{0.03}$ & $0.61^{0.01}$ & $0.61^{0.07}$ & $0.72^{0.01}$ & $0.78^{0.01}$ \\
ZCP + GRAF + PE & $0.45^{0.03}$ & $0.52^{0.02}$ & $\mathbf{0.59^{0.01}}$ & $\mathbf{0.51^{0.04}}$ & $0.55^{0.02}$ & $0.62^{0.01}$ & $\mathbf{0.66^{0.05}}$ & $\mathbf{0.75^{0.02}}$ & $\mathbf{0.79^{0.01}}$ \\
ZCP + GRAF + OH + PE & $0.45^{0.03}$ & $0.52^{0.02}$ & $\mathbf{0.59^{0.01}}$ & $\mathbf{0.51^{0.04}}$ & $\mathbf{0.55^{0.02}}$ & $\mathbf{0.62^{0.01}}$ & $\mathbf{0.66^{0.05}}$ & $\mathbf{0.75^{0.02}}$ & $\mathbf{0.79^{0.01}}$ \\
\end{tabular}
    \end{table}\begin{table}
    \small
    \addtolength{\tabcolsep}{-0.2em}
    \centering
    \caption{Results for various tasks of the TNB101-micro benchmark. Average and standard deviation of Kendall tau over 50 independent runs. Bold values indicate the best results and those that are not statistically different from them.}
    \vskip 0.15in
    \begin{tabular}{r|ccc}
dataset & \multicolumn{3}{|c}{segmentsemantic} \\
train\_size & 32 & 128 & 1024 \\
\hline
OH & $0.42^{0.07}$ & $0.64^{0.03}$ & $0.79^{0.01}$ \\
OH + FP & $0.62^{0.03}$ & $0.69^{0.01}$ & $0.78^{0.01}$ \\
GRAF & $\mathbf{0.68^{0.03}}$ & $0.75^{0.02}$ & $0.81^{0.01}$ \\
GRAF + FP & $\mathbf{0.68^{0.03}}$ & $0.74^{0.02}$ & $0.81^{0.01}$ \\
GRAF + OH & $\mathbf{0.68^{0.03}}$ & $\mathbf{0.75^{0.02}}$ & $0.82^{0.01}$ \\
GRAF + OH + FP & $\mathbf{0.68^{0.03}}$ & $\mathbf{0.75^{0.02}}$ & $\mathbf{0.82^{0.01}}$ \\
\hline
ZCP & $0.62^{0.03}$ & $0.68^{0.01}$ & $0.74^{0.01}$ \\
ZCP + OH & $0.64^{0.03}$ & $0.71^{0.02}$ & $0.77^{0.01}$ \\
ZCP + GRAF & $\mathbf{0.68^{0.03}}$ & $0.74^{0.01}$ & $0.80^{0.01}$ \\
ZCP + GRAF + OH & $\mathbf{0.68^{0.03}}$ & $\mathbf{0.75^{0.02}}$ & $0.81^{0.01}$ \\
\hline
OH + PE & $0.45^{0.05}$ & $0.61^{0.03}$ & $0.79^{0.01}$ \\
OH + FP + PE & $0.63^{0.03}$ & $0.70^{0.02}$ & $0.79^{0.01}$ \\
GRAF + PE & $\mathbf{0.68^{0.03}}$ & $0.75^{0.02}$ & $0.81^{0.01}$ \\
GRAF + FP + PE & $\mathbf{0.68^{0.03}}$ & $0.75^{0.02}$ & $0.81^{0.01}$ \\
GRAF + OH + PE & $\mathbf{0.68^{0.03}}$ & $\mathbf{0.75^{0.02}}$ & $\mathbf{0.82^{0.01}}$ \\
GRAF + OH + FP + PE & $\mathbf{0.68^{0.03}}$ & $\mathbf{0.75^{0.02}}$ & $\mathbf{0.82^{0.01}}$ \\
\hline
ZCP + PE & $0.63^{0.02}$ & $0.69^{0.01}$ & $0.75^{0.01}$ \\
ZCP + OH + PE & $0.64^{0.03}$ & $0.71^{0.02}$ & $0.78^{0.01}$ \\
ZCP + GRAF + PE & $\mathbf{0.68^{0.03}}$ & $0.74^{0.01}$ & $0.80^{0.01}$ \\
ZCP + GRAF + OH + PE & $\mathbf{0.68^{0.03}}$ & $\mathbf{0.75^{0.02}}$ & $0.81^{0.01}$ \\
\end{tabular}
    \end{table}%
